Parallelize Over Data Particle Advection: Participation, Ping Pong Particles, and Overhead

Particle advection is one of the foundational algorithms for visualization and analysis and is central to understanding vector fields common to scientific simulations. Achieving efficient performance with large data in a distributed memory setting is notoriously difficult. Because of its simplicity and minimized movement of large vector field data, the Parallelize over Data (POD) algorithm has become a de facto standard. Despite its simplicity and ubiquitous usage, the scaling issues with the POD algorithm are known and have been described throughout the literature. In this paper, we describe a set of in-depth analyses of the POD algorithm that shed new light on the underlying causes for the poor performance of this algorithm. We designed a series of representative workloads to study the performance of the POD algorithm and executed them on a supercomputer while collecting timing and statistical data for analysis. We then performed two different types of analysis. In the first analysis, we introduce two novel metrics for measuring algorithmic efficiency over the course of a workload run. The second analysis was from the perspective of the particles being advected. Using particle centric analysis, we identify that the overheads associated with particle movement between processes (not the communication itself) have a dramatic impact on the overall execution time. In the first analysis, we introduce two novel metrics for measuring algorithmic efficiency over the course of a workload run. The second analysis was from the perspective of the particles being advected. Using particle-centric analysis, we identify that the overheads associated with particle movement between processes have a dramatic impact on the overall execution time. These overheads become particularly costly when flow features span multiple blocks, resulting in repeated particle circulation between blocks.

==> sections/3_model.tex <==
\section{Theoretical Considerations}
\label{sec:model}
This section describes the framework used to analyze the execution time for a parallel particle advection workload.
\S~\ref{subsec:model:algorithm} describes the algorithm used in this study. 
Following this we provide a theoretical foundation for the imbalance on particle advection methods from two different viewpoints: a rank-based perspective (\S~\ref{subsec:model:rank}) and a particle-based perspective (\S~\ref{subsec:model:particle}).
From a rank-based perspective, the total execution time depends on the process that has the longest execution time. From a particle-based perspective, the total execution time depends on the individual particle that takes the longest time to terminate.
Each viewpoint provides different types of insights into the nature of the problem and provides a basis for performing analysis.


\subsection{Particle advection algorithm}
\label{subsec:model:algorithm}

\input{sections/algorithm}

Algorithm~\ref{pvalgo} contains the pseudocode for performing parallel particle advection used in this paper.
It uses the parallelize over data (POD) scheme where the data blocks are spatially partitioned across a set of processes. Each rank performs the advection for each particle that passes through the block it is assigned. 
During \Icolor{initialization}, each rank assigns the particles contained in the local block to a variable called ActiveQueue (Line~\ref{pvalgo:I1}) and then a global count of the number of particles across all processes is computed (Line~\ref{pvalgo:I2}).

Following initialization, the algorithm executes a while loop until all of the particles terminate or exit the global bounds of the data. The while loop consists of two phases: computation and communication.
%
%Each process has a local queue of particles that exit the local data ($P_{out}$ on Line~\ref{pvalgo:EO1}), and $N_T$, a counter for the number of locally terminated particles (Line~\ref{pvalgo:EO2}.
%

The computation phase is performed if the rank has any work.
If the ActiveQueue is not empty, a particle advection kernel is \BOcolor{readied} with the set of particles (Line~\ref{pvalgo:BO1}).
Execution of the kernel will advance each particle by solving the differential equation using a Runge-Kutta 4 (RK4) solver~\cite{NumericalRecipesInC} to compute the path (Line~\ref{pvalgo:A1}).
Each particle is \Acolor{advected} until a termination criterion is met (i.e., the maximum number of iterations, or the particle enters a zero-velocity region-- a sink), or it exits the spatial domain of the data block.
In the code, when a particle is advected towards the boundary of a block, the RK4 method will fail because not all of the samples for the specified step size can be computed.
For each particle near the boundary, a binary search algorithm is used to reduce the step size to within epsilon of the block boundary. Then a small Euler step is taken to push the particles in $P_{out}$ into the neighboring block (Lines~\ref{pvalgo:A2}-~\ref{pvalgo:A4}).
\ken{As I recall, the discussion of the boundary backoff was added to the paper because we thought it was a major source of overhead from ping pong particles. After more inspection, we found this to be not the case. Should we just remove all discussion of this boundary backoff? It seems weird to introduce readers to something they normally wouldn't think about only to tell them that it doesn't matter.}
Next, at the \EOcolor{end} of advection, the particles exiting the block, $P_{out}$, and the number of terminations are extracted from the advection Result (Lines~\ref{pvalgo:EO1},~\ref{pvalgo:EO2}) and the ActiveQueue is cleared (Line~\ref{pvalgo:EO3}).


Following computation, the \CWcolor{communication} phase is performed using asynchronous message passing with MPI~\cite{mpi40}.
The first step is to send particles in the $P_{out}$ queue to their destinations. The destination rank can be determined from the location of each particle in $P_{out}$. The particles being sent to each destination are bundled together and sent using the asynchronous \texttt{MPI\_Isend}  call (Line~\ref{pvalgo:C1}).
The second step is to update the global counter for the locally terminated particles (Line~\ref{pvalgo:C2}).
If $P_{out}$ is empty or $N_{term}$ is zero, then the operations are both no-ops.
The third step (Line~\ref{pvalgo:C3}) is to receive any incoming particles that have been sent by other ranks. This is done using \texttt{MPI\_Iprobe}, which will indicate if any messages have arrived from other ranks.
If any messages have asynchronously arrived, the \texttt{MPI\_Irecv} call is used to receive them. These incoming particles are added to the ActiveQueue (Line~\ref{pvalgo:C4}) for processing during the next iteration of the loop.





\subsection{Rank centric model}
\label{subsec:model:rank}


In this section, we describe the model for the execution time of the particle advection from a process or rank-centric perspective.
Using the terminology in previous works~\cite{Peterka2011:IPDPS, Pugmire:HPV}, each iteration of the while loop (Lines~\ref{pvalgo:whileBegin}-~\ref{pvalgo:whileEnd} in Algorithm~\ref{pvalgo}) is called a \emph{round}.
In each round, a group of particles is advected and communicated between different ranks. For a specific rank $r$ that takes $N_r$ rounds to complete, the execution time, $T_r$ can be formulated as:

\begin{dmath} 
T_r = \Icolor{$I_{r}$}+ \sum\limits_{i=1}^{N_r} \left [ \BOcolor{$BO_r^{i}$}+\Acolor{$A_{r}^i$}+\EOcolor{$EO_r^{i}$}  +\CWcolor{$C_{r}^i+W_{r}^i$} \right ] \\ 
\label{model:eq1}
\end{dmath}

\begin{dmath} 
T_r = \Icolor{$TI_{r}$}+ \sum\limits_{i=1}^{N_r} \left [ \BOcolor{$TBO_r^{i}$}+\Acolor{$TA_{r}^i$}+\EOcolor{$TEO_r^{i}$}  +\CWcolor{$TC_{r}^i+TW_{r}^i$} \right ] \\ 
\label{model:eq1}
\end{dmath}

\begin{dmath} 
T_r = \Icolor{$T(I_{r})$}+ \sum\limits_{i=1}^{N_r} \left [ \BOcolor{$T(BO_r^{i})$}+\Acolor{$T(A_{r}^i$)}+\EOcolor{$T(EO_r^{i})$}  +\CWcolor{$T(C_{r}^i)+T(W_{r}^i$)} \right ] \\ 
\label{model:eq1}
\end{dmath}

\begin{dmath} 
\label{model:eq1}
T_r = \Icolor{$\tau I_{r}$}+ \sum\limits_{i=1}^{N_r} \left [ \BOcolor{$\tau BO_r^{i}$}+\Acolor{$\tau A_{r}^i$}+\EOcolor{$\tau EO_r^{i}$}  +\CWcolor{$\tau C_{r}^i+\tau W_{r}^i$} \right ] \\ 
\end{dmath}

% Try to use T notation (For testing)
\begin{dmath}
T_r = \Icolor{$T_I(r)$}+ \sum\limits_{i=1}^{N_r} \left [ \BOcolor{$T_{BO}(r,i)$}+\Acolor{$T_A(r,i)$}+\EOcolor{$T_{EO}(r,i)$} +\CWcolor{$T_{C}(r,i)$} + \CWcolor{$T_{W}(r,i)$} \right ]
\end{dmath}

\begin{dmath}
T_r = \Icolor{$TI(r)$}+ \sum\limits_{i=1}^{N_r} \left [ \BOcolor{$TBO(r,i)$}+\Acolor{$TA(r,i)$}+\EOcolor{$T{EO}(r,i)$} +\CWcolor{$TC(r,i)$} + \CWcolor{$TW(r,i)$} \right ]
\end{dmath}


\noindent
The definition of terms for a particular rank $r$ at the $i^{th}$ round are described below. For clarity, the line numbers specified below are in reference to those in  Algorithm~\ref{pvalgo}.
\begin{itemize}
    \item \Icolor{$I_{r}$} is the time for initialization. (Lines~\ref{pvalgo:I1}-~\ref{pvalgo:I2})
    
    \item \BOcolor{$BO_r^{i}$}  denotes ``begin overhead'', the overhead required to initialize a worklet with a batch of particles. This overhead includes the time to select active particles and create the necessary data structures within the kernel for particle advection. (Line~\ref{pvalgo:BO1}).
    
    \item \Acolor{$A_{r}^i$} denotes the time to advect a batch of particles until they terminate or leave the data block during round $i$. As described above in \S~\ref{subsec:model:algorithm}, for particles leaving the data block, the step size is reduced to place the particle within epsilon of the block boundary, and then an Euler step is taken to push it outside the data block (Lines~\ref{pvalgo:A1}-~\ref{pvalgo:A4}).
    
    \item \EOcolor{$EO_r^{i}$} denotes ``end overhead'', the overhead required to determine the status of each particle (i.e., determining the particles that leave the block and those that terminate) and clearing the ActiveQueue (Lines~\ref{pvalgo:EO1}-~\ref{pvalgo:EO3}).
    
    \item \CWcolor{$C_{r}^i$} represents the time to exchange particles and update the global counter. This includes serializing the particles into a message, sending it over the network and deserialization. (Lines~\ref{pvalgo:C1}-~\ref{pvalgo:C3}).
    \item \CWcolor{$W_{r}^i$} represents the time spent when a rank has no work to perform. When using asynchronous communication this term is difficult to compute, so we merge \CWcolor{$C_{r}^i$} and \CWcolor{$W_{r}^i$} into a single term, \CWcolor{$CW_{r}^i$} that captures the communication and wait time.
\end{itemize}

%\dave{I wonder if this paragraph should be moved to the results section.}
%It is observed that $EO_r^{i}$ is not influenced by the length of the particle trajectories (unlike $A_{r}^i$), however, it can be impacted by the number of particles that exit the domain boundary. This is because each particle that exits the data block necessitates extra processing to move the particle to the boundary.

The total execution time for the entire
workload, $T_{total}$ is the 
execution time for the rank with the longest execution time.
\begin{equation}
   T_{total} = \max (T_1,  \ldots, T_{r}) \nonumber
\end{equation}

\begin{comment}
\label{subsec:model:rank}
\begin{figure}[ht]
\centering
\subfigure[Sync MPI]{
\includegraphics[width=65mm]{./figs/GantCharts/gantt_chart_rank_visreader_test_astro_data_sync.png}
}
\subfigure[Async MPI]{
\includegraphics[width=65mm]{./figs/GantCharts/gantt_chart_rank_visreader_test_astro_data_async.png}
}
\caption{Example Gantt charts of particle advection for the Supernova data set. There are $8$ data blocks (one data block per rank), $5000$ particles per rank and $2000$ advection steps per particle. }
%\ken{I note that some Gantt charts, like this one, use pink as the "comm/wait" time whereas others (the per particle charts) use white as "comm/wait". These should be made consistent. I personally think white makes the most sense for "comm/wait". Can we switch the colors for "comm/wait" and "other"?}
%\ken{I don't understand this argument. Lots of charts include an "other" category, and it is rarely if ever colored the background color. Making the processor idle time the background color makes the most sense.}
% Jay: figure is updated, the style of subsequent figures will be udpated soon

\label{fig:model:rankgantt}
\end{figure}


Figure~\ref{fig:model:rankgantt} illustrates a proof of concept for Gantt charts of each computing rank. When using synchronous MPI communication, each rank has same number of rounds; however, the number of rounds are different among ranks when using the asynchronous MPI protocol for POD.
We cannot compare the workload for each round between different processes discussed in related works~\cite{nouanesengsy2011load}. \ken{Uh, what?}

Gantt charts based on the rank-centric model are intuitive for showing the workload balance between different ranks.
For example, Figure~\ref{fig:model:rankgantt} shows that the system starts balanced, but the load becomes concentrated on ranks $0$ and $2$ by the end.
Load imbalance shown by these these Gantt charts indicates that particles are gathered to a subset of blocks, and the associated ranks need to process more particles than others.
However, it is hard to quantify the unbalanced workload using the rank-centric model. In particular, for particles having the same number of advection steps, we might ask why some particles have longer execution time than others during the particle advection. This question drives us to consider the workload of particle advection from the perspective of each particle.
\end{comment}

\subsection{Particle centric model}
\label{subsec:model:particle}

% Do not use this figure, maybe disucss the wait time at the evaluation section
%\begin{figure}[ht]
%\centering
%\label{fig:model:particle:gantt1}
%\includegraphics[width=70mm]{./figs/ParticleGantt/particle_gant_astro_8ranks.png}
%\caption{
%Gantt charts for a particle with the longest execution time in the Supernova data set.
%The colored bar means that the particle is in the advection call. Different colors mean that the particle is located in different ranks. White regions represent the time period when the particle is not being processed (e.g., it is waiting in a queue or experiencing other overhead). The blue dashed line labels the moment before particle communication operation, and the red dashed line labels the moment when all packets of corresponding particle group are received by dedicated rank.
%}
%\label{fig:particle_gantt}
%\end{figure}

As a particle is advected throughout a given dataset, it traverses through a sequence of blocks. Given a particle with index $p$ that travels through a total of $N_p$ blocks (i.e., $B_1$, \ldots , $B_{N_p}$), the execution time, $T_p$ can be formulated as:

\begin{equation}
T_p = \Icolor{$I_{p}$}+ \sum\limits_{i=1}^{N_p} \left [ \BOcolor{$BO_p^{i}$}+\Acolor{$A_{p}^i$}+\EOcolor{$EO_p^{i}$}  +\CWcolor{$C_{p}^i+W_{p}^i$} \right ]
\label{model:eq2}
\end{equation}

% Try to use T (For testing)
\begin{dmath}
T_p = \Icolor{$T_I(p)$}+ \sum\limits_{i=1}^{N_p} \left [ \BOcolor{$T_{BO}(p,i)$}+\Acolor{$T_A(p,i)$}+\EOcolor{$T_{EO}(p,i)$} +\CWcolor{$T_{C}(p,i)$} + \CWcolor{$T_{W}(p,i)$} \right ]
\end{dmath}

The terms in the particle centric model are similar to those of the rank centric model. As such we describe them with much less detail. Again, the line numbers refer to those in Algorithm~\ref{pvalgo}.

\begin{itemize}
    \item \Icolor{$I_p$} is the time for initialization of the group of particles where $p$ begins (Lines~\ref{pvalgo:I1}-~\ref{pvalgo:I2}).
    \item \BOcolor{$BO_p^{i}$} (Line~\ref{pvalgo:BO1}) and \EOcolor{$EO_p^{i}$} (Lines~\ref{pvalgo:EO1}-~\ref{pvalgo:EO3}) represent the begin overhead and end overhead, respectively, of processing the group where particle $p$ is located when being processed in the $i^{th}$ block sequence.
    \item \Acolor{$A_p^{i}$} represents the time for computing the paths for the particle group containing particle $p$ (Lines~\ref{pvalgo:A1}-~\ref{pvalgo:A4}).
    \item \CWcolor{$C_p^{i}$} represents the time for communicating particle $p$, along with any other particles in the group (Line~\ref{pvalgo:C1}.
    \item \CWcolor{$W_p^{i}$} represents the time waiting for the next rank to receive particle $p$. For example, when the receiver rank is occupied by another computation task, it can not start to receive the particle sent from other ranks, and particle $p$ needs to wait. As in the rank-centric model (\S~\ref{subsec:model:rank}),  asynchronous communication causes difficulty in separating the wait time from communication time, and so \CWcolor{$C_p^{i}$} and \CWcolor{$W_p^{i}$} are merged into a single term, \CWcolor{$CW_p^{i}$} (Lines~\ref{pvalgo:C1}-~\ref{pvalgo:C4}) that captures the communication and wait time.
\end{itemize}

The total execution time for the entire
workload, $T_{total}$ is simply the 
execution time for the slowest particle.

\begin{equation}
   T_{total} = \max (T_1, T_2, \ldots, T_p, \ldots) \nonumber
\end{equation}

It is important to note that Algorithm~\ref{pvalgo} processes groups of particles together. This is desirable to keep processors busy and to minimize the amount of communication. As such, particles are processed in groups, and the execution time is a function of the time to compute the particles in the same group as particle $p$.

% Single factor may not necessary casue the unbalance

%\begin{enumerate}

    %\item Number of traversed block is large. 

    %\item Large batch size along particle advection path. A dedicated particle will passes through a series of blocks during advection, if workload along this path is significantly larger than others, this particle needs more cost to complete its execution compared with other particles. For two particle that have same number of traversed block among its advection path, if we assume the advection steps are distributed among each traversed block in a same pattern, the particle with a large block size on its path can cause a long particle advection time and associated begin/end overhead. In addition, since the process holding the receiving process might be occupied, the targeted particle need to wait for the completion of the particle advection in the previous round to use the corresponding computation resource. Therefore, the large batch size along path can increase both accumulated advection time and wait time. 
    % in order to complete this path, how much extra advection operaion need to be executed, larget batch size indicates more overhead

    %\item Accumulated advection time is long. When there is a large particle batch size (the number of particles processed by a process when passing a specific block), the advection time can increase. For a particle passing through a dedicated block, 
    
    %motorcycle gang.
    
    %\item Waiting time is long. When the current process receives particles, the previous particle batch might still occupy the computing resources. Newly arrived particles need to wait for the completion of the particle advection in the previous round to use the corresponding computation resource. 
    
    %\item Overheads are large. When particles traverse a large number of blocks in different ranks, the number of rounds for rank ($N_r$) or the number of traversed compute rank per particle ($N_p$) can be a large number. Therefore, 

    % \item More?
%\end{enumerate}

% add several sentences here, more np, more accumulated Ap large group gang size for particular particle during its advection path b1b2...bNp more no, what effects, if bnp have large gang, what effects

%Figure~\ref{fig:particle_gantt} shows the longest execution particle for the Supernova data set running on $8$ ranks using asynchronous MPI communication for the proof of concepts. There is one data block per rank, $5000$ particles per data block, and $1000$ steps per particle. The solid colored bar represents the particle advection time, and the blue dashed line labels the moment when communication starts. The red dashed line labels the moment when the particle is received by the dedicated compute rank. It is worth noting that the asynchronous communication protocol we adopted in this work divide whole group of particles into multiple packets when sending a bunch of particle to a dedicated rank. The dedicated compute rank start to process the corresponding bunch of particle only when all packets are arrived.
%\dave{Address this re: the probe implementation.}

% syncroubous protocol is comparatively simple, using allreduce to get the message size(metadata) each time, then go through each message using original send recv to transfer data

%with the following sequence:

%\begin{multline}
%I_iBO_{i,1} A_{i,1} EO_{i,1} S_{i,1}Q_{i,2}BO_{i,2}A_{i,2}EO_{i,2}S_{i,2}... \\
%Q_{i,N_i-1}BO_{i,N_i-1}A_{i,N_i-1}EO_{i,N_i-1}S_{i,N_i-1} \\
%Q_{i,N_i}BO_{i,N_i}A_{i,N_i}EO_{i,N_i}
%\end{multline}
%

%\noindent
%where:
%\begin{itemize}
%    \item $I_i$ represents 
%    the initialization work for a particle, i.e., queueing up the particle
%    on the correct compute
%    rank that has the block that contains its seed 
%    location.
%    \item $BO_{i,j}$ represents the overhead 
%     for particle $i$ to begin advection on its $j^{th}$
%     compute rank (``BO'' means ``begin overhead'').
%    \item $A_{i,j}$ represents the advection steps
%    taken by particle $i$ while on its $j^{th}$
%    compute rank.
%    \item $EO_{i,j}$ represents the overhead 
%     for particle $i$ to end advection on its $j^{th}$
%     compute rank (``EO'' means ``end overhead'').
%    \item $S_{i, j}$ represents the process of sending particle from its $j^{th}$ compute 
%    rank to its $(j+1)^{st}$ compute rank,
%    i.e., encoding it as a message, sending
%    it over a network, and decoding the message.
%    \item $Q_{i,j}$ represents the time  particle $i$
%    spends waiting on its $j^{th}$ compute rank
%    before advection begins.
%\end{itemize}

%If $T$ represents  the time for each execution phase, 
%then the total time for a given
%particle $i$ to advect is:

%\begin{multline}
%   T(i) = T(I_i) + 
%   \sum_{2}^{N_i} T(Q_{i,1})  +
%   \sum_{1}^{N_i} T(BO_{i,1})  +
%   \sum_{1}^{N_i} T(A_{i,1})  + \\
%   \sum_{1}^{N_i} T(EO_{i,1})  +
%   \sum_{1}^{N_i-1} T(S_{i,1}) 
%\end{multline}




==> sections/5-1_results.tex <==
\section{Results}
\label{sec:results}
% Outline-
% - Rank centric
% - - Time, weak scaling.
% - - Gantt charts
% - - table of percentages ** Add **
% - - participation rates
% - Particle centric
% - - long particle gantt
% - - ping pong
% - - alive particle statistics



Following the discussion in Section~\ref{sec:model}, the results are collected using both rank-centric and particle-centric modeling.
The code was instrumented to collect data for the coefficients in both Equations~\ref{model:eq1} and~\ref{model:eq2}. 

The rank-centric data was collected by recording a time-stamp each time the algorithm transitioned from one state to another. For example, during each round timestamps were collected for the begin and start of each round as well as for subtasks within the round (e.g., advection ($A$), communication ($C$), etc). Timestamps were synchronized so that comparisons across all of the ranks is possible.

\begin{figure}[ht]
\centering
\includegraphics[width=3in]{./figs/advectTimingDetail}
\caption{Detail of timings for Eq2.}
\label{fig:advectDetailTimings}
\end{figure}

\dave{Insert text to describe how timings were captured in the figure above.}

The particle-centric data was collected in two different ways. The first was to capture bulk data for all of the particles. This included the number of blocks a particle traverses, termination time and reason for termination.
Second, we provided the ability to specify a unique id to collect detailed information for a single particle.  In this mode, each rank will check the particles being processed and record additional information for the particle. In addition to recording the bulk data listed above, it records which ranks are traversed and  timestamps to record when a particle is communicated, when it it received and when it processed after communication.

\begin{figure}[ht]
\centering
\includegraphics[width=3in]{./figs/particleFlowDiagram}
\caption{Particle-centric state diagram. \dave{Also needs to address the wait due to  multiple packets.}}
\label{fig:particleFlowDiagram}
\end{figure}

All of the collected data was held in memory and written to log files after algorithm execution was complete. To verify that our instrumentation does not significantly alter runtime behaviour, the experiments were run both with and without collecting this data. We found that the overhead for collecting this data was at most $2.8\%$.
%Data from slide 162



\subsection{Rank-centric Analysis}
\label{results:rank-centric}

%\begin{figure*}[ht]
%\centering
%\includegraphics[width=\linewidth]%{./figs/summary_timings}
%\caption{Summary timings.}
%\label{fig:summary_times}
%\end{figure*}


\begin{figure*}[ht]
\centering
\includegraphics[width=181mm]{./figs/ScaleEfficiency/all_exec_eff_time.pdf}
\caption{The first row of figures show execution time of the particle advection filter for all evaluated datasets with different number of ranks. The log scale (the base value is 2) is adopted for both $x$ and $y$ axis. The second row of figures show weak scaling efficiency of all evaluated data sets with different number of ranks. 
%\ken{The x-axis should be labeled (\# of ranks).}
%\ken{The y axis for efficiency should all be scaled from 0 to 1.}
% Jay, the x label and y axis is updated
}
\label{fig:results:scale}
\end{figure*}


Figure~\ref{fig:results:scale} shows the total execution time for a weak scaling run on each of the five data sets. As described above, we maintain a fixed seed count of $5000$ for each data block, and assignment of one block per rank. As such, the number of ranks and the number of blocks is the same. The number of steps varies between $50$ and $2000$.

The weak scaling efficiency for each experiment is shown in (a.2) to (e.2) in Figure~\ref{fig:results:scale}.
The weak scale efficiency for a run with $N$ ranks is defined as the ratio $T(N)/T(8)$. $T(8)$ is time to execute an experiment with $8$ ranks (the lowest level of concurrency) and $T(N)$ is the time to execute an experiment with $N$ ranks.
This is consistent with a unit-cost-based efficiency \cite{Moreland2015:ISC} using the 8-rank case as a base and recognizing that the problem size increases proportionally to the number of ranks.
Perfect scaling gives an efficiency value of $1$ for all $N$.
The weak scaling efficiency over all experiments significantly declines as the number of ranks increases, even for cases that are ideal for the POD algorithm (i.e. Tokamak and Synthetic).
Additionally, the efficiency drops as the number of advection steps grows and is particularly pronounced in the Supernova and CloverLeaf3D data sets.


Gantt charts provide an effective way to understand the activity of each rank over the course of the execution.
Figure~\ref{fig:results:gantt} shows Gantt charts for a workload consisting of 128 ranks and 2000 steps for each dataset.
In these figures, blue regions represent the advection time, the pink regions account for both wait time and communication time, and the white region represents other associated overhead. 
%\ken{I would call that pink, not red. Also, see my comment in the caption of Figure \ref{fig:model:rankgantt}.}
These charts provide an overview of the overall balance of work among the ranks and give insight into the overall scalability.
The Gantt charts for the Tokamak, Hydraulics, and Synthetic datasets appear to have more balanced workloads.
Conversely, the Gantt charts for Supernova and CloverLeaf3D clearly illustrate that the reason for long execution times is that a relatively small number of ranks have much more work, which results in poor efficiency.
\dave{A big part of the problem is that the particle path has to be executed in order -- the amount of parallelism is constrained.}
%In particular, the Gantt charts for Supernova and CloverLeaf3D data sets reveal the presence of ranks with a significantly longer execution time than others. These ranks with a long execution time cause the work imbalances and low weak scale efficiency. Conversely, Gantt charts from the remaining three data sets show more balanced workloads throughout the particle execution. To quantitatively assess the varying degree of each rank's involvement in particle advection processing over time, a suitable metric needs to be developed further.
\dave{Insert references back to equation 1.}








To  quantify the overall efficiency, we introduce a simple metric called \emph{rank participation} to illustrate the overall performance of the algorithm over the course of execution.
Rank participation is defined as the fraction of ranks actively doing work.
Specifically, if $N_T$ is the total number of ranks in the parallel job and $N_A$ is the number of ranks actively doing work, then the rank participation is $N_A/N_T$.
The rank participation can be measured instantaneously or integrated over the execution of the algorithm.
A rank participation of $1$ represents a perfectly load balanced operation whereas a small rank participation of $1/N_T$ means one rank is working while the rest remain idle.



%\begin{figure*}[ht]
%\centering
%\includegraphics[width=\linewidth]%{./figs/fusion_astro_64_gantt_RP}
%\caption{Representative Gantt chart and associated rank participation chart}
%\label{fig:summary_gantt}
%\end{figure*}

\begin{figure*}[ht]
\centering
 
\includegraphics[width=180mm]{./figs/GantCharts/rank_gantt_all.png}
\caption{Gantt charts for evaluated data sets when there are $128$ ranks and $2000$ advection steps.}
\label{fig:results:gantt} 
\end{figure*}





\begin{figure*}[ht]
\centering
\label{fig:scale}  \includegraphics[width=180mm]{./figs/Participation/rank_participation_all.pdf}
\caption{Participation rates when there are $128$ ranks and $2000$ advection steps for evaluated data sets.}
\label{fig:results:pr}
\end{figure*}

%\dave{participation rate images: add charts with more ranks/steps. Can normalize the runtime so that multiple runs can be put in 1 plot.}
% Jay: the exeuction time is a little bit different for different configurations, maybe we need double check about the proper visualization results, I tested 128 blocks with 50 steps, which has similar trend with current results. 

Figure~\ref{fig:results:pr} shows the rank participation values for the same runs shown in Figure~\ref{fig:results:gantt} ($128$ blocks and $2000$ advection steps).
%\ken{It just occured to me that the phrase ``rank participation rate'' is used several times. Is rank participation really a rate? A rate generally compares things of different units, which is not the case here. I suggest removing rate and just say ``rank participation''.}
% Jay: we updated it into rank participation and aggregated rank participation
The rank participation curve provides a straightforward view of the number of ranks actively engaged as the algorithm progresses. We note that a rank is marked as participating when it is performing any of the following tasks: $A$, $BO$, $EO$ and $C$ from Equation~\ref{model:eq1}. And conversely, a rank is marked as not participating when it is idle (task $W$ from Equation~\ref{model:eq1}.)
The participation rate charts highlight the problems with efficiency for the Supernova and CloverLeaf3D datasets as there is a dramatic drop in participation at the outset of the execution.
The Tokamak and Synethetic datasets exhibit relatively consistent and steady participation rates over the course the execution while the Hydraulics dataset lies somewhere in the middle.

We further compute the \emph{aggregated rank participation} over the course of a run by integrating the participation rank curve (the area under the rank participation curve) across a normalized time axis. If all ranks were engaged across the entirety of the run, the aggregated participation rate would be $1.0$. 
The aggregated rank participation values are shown in Figure~\ref{fig:summary_RP} for all of the experiments examined in our study. All of the runs for a given dataset are shown as a subplot.
The curves in each subplot track the aggregated rank participation for a run at a given level of parallelism as a function of the number of advection steps.
As an example, the purple line in the Tokamak subplot shows the aggregated rank participation running on $128$ ranks and advection steps of 50, 100, 500, 1000, and 2000.
Plotting these metrics provides insight into the scalability of the algorithm across different datasets and workloads. 
Specifically, Tokamak and Synthetic data have high average rank participation values, whereas Supernova and CloverLeaf3D exhibit lower participation values when the number of ranks increases from $8$ to $128$. The average participation rates are more sensitive to the number of ranks for Supernova and CloverLeaf3D data sets compared to other datasets. 
%\dave{A lot more graphs are available for participation rate. I think more would explain what is going on. Participation rate and weak scaling are related so these need to be discussed together.}
% Jay: we added weak scaling efficiency to further explain the results

\begin{figure*}[ht]
\centering

\includegraphics[width=180mm]{./figs/Participation/rank_participation_gather_all.pdf}
\caption{Aggregated participation rates across all evaluated datasets.  
%\dave{X axis is Total number of advection steps, OR, put a dot on each experiment.} %\dave{change plot axes title to aggregated.}
}
% Jay, x y axes are updated and the dot is added into the figure
\label{fig:summary_RP}
\end{figure*}



\subsection{Particle-centric Analysis}
\label{subsec:pstatus}
Rank-centric analysis provides a broad perspective of algorithm efficiency.
Evaluation results shown above in Section~\ref{results:rank-centric} reveal the degrees of workload imbalance across evaluated data sets and workloads.
It lacks, however, the ability to provide a clear insight into the barriers to scalability.
To probe more deeply into scalability issues we explore the model analysis in section~\ref{subsec:model:particle} and study the performance from a particle-centric perspective. 



%\subsubsection{Oldest particle analysis}
\subsubsection{Long running particle analysis}

Algorithm execution time is determined by the particle with the maximum execution time (Equation~\ref{model:eq2}). 
Because of this, investigating particles with long execution time can offers insights into algorithm performance.
Collecting the data from Equation~\ref{model:eq2} for each particle would introduce significant overheads. To avoid this problem we collect data on a representative particle with a long execution time.
Determining a representative particle is straightforward. When the algorithm is run we record the ID of the last particle that terminates. We then re-run the algorithm and collect data only on the particle with that specified ID.
In practice, when using asynchronous communication, the particle with the longest execution time is not always the same, but the execution times are similar enough that it provides an accurate representation of the longest running particle.



%\dave{Do we want to show and discuss this table?}
The data in Table~\ref{tab:long_particle} shows data collected from the long running particle for the 128 rank cases of $2000$ steps over each dataset.
The values for each variable in Equation~\ref{model:eq2} are shown as a percentage of the total time for the particle. 
\ken{I'm reading this paper out of order, so I might have just missed it, but is it described how the terms of Equation \ref{model:eq2} are measured? I expect $A$ is everything in the advection loop, and $BO$ and $EO$ are the things before and after this loop, respectively. How do you differentiate when a particle is communicating and when it is waiting?}
\dave{I think we need some sort of graphic that describes what we are timing. Perhaps a block or state diagram.}
\james{This large table only gets one small paragraph of explanation. Further, there doesn't seem to be a takeaway here. What am I supposed to understand from this analysis? Just emphasizing that your model has different components? Maybe a forward reference to where you explain the differences in advection vs wait time for different step sizes? Then, the next few graphs only talk to the 2000 step case. Is the 1000 step important here, if so, that should be a finding in the text. Next, a refresher on the equation should be in the table or the text, that was many sections ago. Lastly, without expanding the explanation quite a bit, I think the other graphics are more compelling, so this could be skipped.}

\input{sections/percentage_table}


\begin{figure*}[ht]
\centering
\includegraphics[width=180mm]{./figs/ParticleLongExec/particle_gantt_five_datasets_red_wait.pdf}
\caption{Gantt chars of the particle with long execution time for evaluated data sets when there are $128$ blocks and $2000$ advection steps. The pink color represents wait and communication time. Other colored bars represent the advection time. In particular, advection in different blocks is represented by one color chosen from the viridis color map. The white colored slot during the particle execution between the pink colored bar and other colored bars represents other overhead.}
\label{fig:particle_long_exec}
\end{figure*}


%\james{This figure would be much more compelling at full page width. Also, the zoomed in view is not showing anymore.}
% Jay: the Figure9 is updated to full page width
\dave{We need to provide a clear explanation of what we are recording. syncronized time stamps are set on a particle whenver it goes into the worklet.Advect(). Explain what is going on in the white space.}
Figure~\ref{fig:particle_long_exec} shows Gantt charts of an individual particle for a workload of 128 blocks and 2000 advection steps for all datasets.
The bars in the chart are colored by the rank ID where the particle resides. The width of the bar indicates how long the particle is on a given rank for advection. The spaces between each bar indicate that a particle is waiting to be processed (e.g., being communicated, waiting in the queue for processing, etc). 
%It is worth noting that these Gantt charts are rendered with limited precision. Very thin bars get inflated to a minimum (pixel) width.
%For instance, in Figure~\ref{fig:particle_long_exec:b}, a zoomed-in view of the Gantt chart for the Hydraulics dataset offers a more detailed perspective.

\begin{figure}[ht]
\centering
\subfigure{
\includegraphics[height=35mm]{./figs/Astro-pingpong}
}
\hspace{5mm}
\subfigure{
\includegraphics[height=35mm]{./figs/Clover-pingpong}
}
\caption{Examples of a particle that ping pongs in the Supernova (left figure) and Cloverleaf3D (right figure) dataset. The long running particles are trapped into a vortex crossing two adjacent data blocks.}
\label{fig:example_pingpong}
\end{figure}

An observation from Figure~\ref{fig:particle_long_exec} is that the particle is repeatedly passed back and forth between two compute ranks. In particular, in the  Supernova and CloverLeaf3D datasets, the stage where the particle is circulating back and forth between ranks takes more than half of the total execution time.
Particles exhibiting this behaviour are shown in Figures~\ref{fig:example_pingpong} for the Supernova and CloverLeaf3D datasets. A vortex exists in each dataset that is near a block boundary that results in particle circulation between the two blocks.
We provide a more detailed analysis and explore methods to alleviate this situation later in Section~\ref{discus:pingpong}.

\dave{Remove the packet-text. Also address the overhead above as setup for talking about the particle gantt charts.}
Another observation stemming from Figure~\ref{fig:particle_long_exec} is the existence of wait time for long running particles. Each time when a tracing particle moves to a new block, it introduces extra wait time and overhead, such as getting particles and small advection steps closing to boundary. The length of accumulated wait time is influenced by configurations of asynchronous MPI protocol used in the study. The associated protocol decompose message into several small packets with fixed length, and the number of alive \texttt{MPI\_Irecv} (termed by ``receivers'' in this study) remains constant during the particle execution. The particles stored in message will be extracted and advected only when all packets are received by a receiver.

Figure~\ref{fig:chage_recv} illustrates accumulated wait time, advection time, and other overhead on average (three runs) for a long running particle.  The Supernova data set is adopted in this experiment, and the number of receivers changes from $64$ to $1024$. There is a tradeoff between accumulated wait time, accumulated advection time, and other overhead. When we use a large number of receivers, such as $1024$, the message will be received within fewer iterations in receivers, resulting in a reduction of accumulated wait time. However, the size of the particle group and the targeted particle increases, leading to more accumulated advection time and other overhead.

\begin{figure}[ht]
\centering
\includegraphics[height=50mm]{./figs/ParticleLongExec/SupernovaChangeRecvs.pdf}
\caption{The accumulated time for different stages of long running time of Supernova data set when there are $128$ blocks and $2000$ steps.}
\label{fig:chage_recv}
\end{figure}


\subsubsection{Particle lifetime analysis}


\begin{figure*}[ht]
\centering
\includegraphics[width=180mm]{./figs/ParticleTermination/particles_all_dots_all.png}
\caption{Scatter plot of particle when they are terminated. There are $128$ ranks and $2000$ advection steps. The $x$ axis represents the ratio of particle active time to the particle advection execution time. The $y$ axis represents the number of traveled blocks for each particle. The denser colored regions represents more number of terminated particles. The larger circle corresponds to a larger accumulated group size when particle terminates.}
\label{fig:particle_scatter}
\end{figure*}

\begin{figure*}[ht]
\centering
\includegraphics[width=180mm]{./figs/ParticleTermination/particles_bars_all.pdf}
\caption{The colored bars represent the number of terminated particles (labeled on the left $y$ axis) when using $128$ ranks and $2000$ advection steps. Different color represents different termination reasons. 
The orange curve represents the number of active particles (labeled on the right $y$ axis) within a specific time slot during the particle execution .}
\label{fig:particle_num}
\end{figure*}


\dave{Should this go before the particle gantt charts? Need to tie these results to Eq 2.}
The previous subsection discusses the execution path of long running particles, while the current subsection presents statistics for all particles. 
During each run, data are collected for each particle. These include the time when a particle terminates, the number of blocks traversed by the particle, and the reason the particle terminated. Reasons for termination are as follows:
\begin{itemize}
    \item Out of bounds: The particle exited the spatial bounds of the dataset.
    \item Zero velocity: The particle enters a sink.
    \item Max step: The maximum number of advection steps is achieved.
\end{itemize}
Figure~\ref{fig:particle_scatter} provides a holistic view of statistics for when particles terminate over each dataset. 
%\dave{insert comment on particle sampling.. Why not Synthetic?}
% Jay, synthetic results are added, and we also added how particles are sampled
We sample the particle with a sample rate of $200$ and scatter associated particle statistics in the figure. In particular, the X axis is the execution time, normalized to 1. The Y axis is the number of blocks traversed by a particle. The color indicates the particle termination reason. The denser color represents more particles terminated in the corresponding region, and a longer diameter of a circle point indicates a larger accumulated group size when a particle terminates.
For the Tokamak data set, the number of traversed blocks remains constant at the half stage of particle execution; the long running particles are mainly caused by the large size of the particle group. The Supernova data set indicates that both the large number of traversed blocks and group size can contribute to the long execution time. Intriguingly, particles terminating at around $60\%$ of execution time, despite sharing a similar number of traversed blocks with the particle terminating at around $100\%$ of execution time, demonstrate a smaller group size and consequently less execution time. In addition, Hydraulics and CloverLeaf3D data sets also indicate that the particles having the longest execution time are caused by a large number of traversing blocks and accumulated group size. These results are aligned with the theoretical consideration discussed in subsection~\ref{subsec:model:particle}.

%\james{The figure associated with this section is not clear. You use the term "available" and "active" interchangeably, which is somewhat confusing. The fact that the color legend should be used from the previous figure was not immediately clear, as it is a standalone figure, not a subfigure. Which y-axis went with which data was not clear. A legend would fix this (though I would not use a blue curve while also using blue bars in the same figure). }
% Jay, figure and associated descriptions are updated


\begin{table}[ht]
\begin{center}
\caption {Percentage of terminated particles with different reasons for $128$ data blocks and $2000$ advection steps.}
\label{tab:long_particle}
\begin{tabular}{llll}
\toprule
Data sets &  Out of bounds & Zero velocity &  Max steps  \\
\midrule
Tokamak  & $2.1\%$  & $69.1\%$ & $28.8\%$  \\
\midrule
Supernova  & $82.5\%$  & $8.5\%$ & $9.0\%$  \\
\midrule
Hydraulics  & $39.6\%$  & $59.0\%$ & $1.4\%$  \\
\midrule
CloverLeaf3D  & $15.1\%$  & $41.9\%$ & $43.0\%$  \\
\midrule
Synthetic  & $26.2\%$  & $12.7\%$ & $61.1\%$  \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


\james{What is the takeaway here? The paragraph describes what we can see, but not what we learn. Short takeaway and a forward reference to the discussion if necessary}
\textcolor{red}{Jay, we added some take away information, maybe need to discuss more}

Figure~\ref{fig:particle_num} further illustrates the number of terminated particles over time. The colored bar represents the number of terminated particles for each time slot, and the blue colored curve represents the number of active particles. For Tokamak, Supernova, and Hydraulics data sets, the number of active particles drops quickly at the early stage of the execution and then decreases gradually till the end of the particle advection. For CloverLeaf3D, the number of alive drops to $100,000$ particles and maintains this level throughout the course of execution.


Experiment results shown in particle-centric analysis reveals why there are different execution time for evaluated data sets with the same workload configurations. For example, there are a few green colored bars for Hydraulics in Figure~\ref{fig:particle_scatter}, which shows that most of the particles are terminated before completing all advection steps. In particular, only $1.4\%$ particles for the Hydraulics data set complete all their advection steps. Therefore, Hydraulics takes less time to complete particle advection compared with other data sets. Although the Supernova data set has $9.0\%$ particles completing all advection steps, it takes longer execution time than the Tokamak data set, which has $28.8\%$ max step particles. This is because the Supernova data set has more particles passing back between adjacent data blocks (illustrated in Figure~\ref{fig:particle_long_exec}), and these particles increase the particle advection's execution time.

%\subsection{Reasons for poor performance}


%\begin{itemize}
%    \item Participation rates.
%    \begin{itemize}
%        \item Story: problem exists, gets worse at scale for many data-sets.
%        \item Gantt charts for 2 cases and participation plot
%        \item Table with percentages
%        \item summary chart: Astro: x= numsteps, y= participation. show lines for 8,16,32,64,128,... (similar to figure 3)
%        \item insert discussion from slides on what to discuss here.
%    \end{itemize}
%    \item why the participation is so bad. Item 1 is ping pong.
%    \item Ping pong
%    \begin{itemize}
%        \item show traces of codes, discuss paterns
%        \item rank and particle gantt charts
%        \item Astro has LOTS of ping pong particles. (rank particle , step charts)
%        \item how it appears / disappears with num blocks. Show gantt chart at 8 ranks, 16, compared to 128. Consider the other charts if needed. (final rank)
%    \end{itemize}
%\end{itemize}


%Two problems exist. participation, ping pong.
%ping pong and number of blocks. astro vs. fusion/synthetic

%Discuss the magnitude. how bad it hurts.


==> sections/5-2_results.tex <==
\clearpage 

\input{sections/percentage_table}

\section{Results: Slowest Particle}
\label{sec:results}
% Outline-
% - Rank centric
% - - Time, weak scaling.
% - - Gantt charts
% - - table of percentages ** Add **
% - - participation rates
% - Particle centric
% - - long particle gantt
% - - ping pong
% - - alive particle statistics



%\subsection{Execution Time Analysis}
The overall execution time for an algorithm is only as fast as the slowest
particle, i.e., the particle that takes the longest
to complete execution.
%
Our analysis of performance begins by considering the time spent for 
the slowest particle over a variety of configurations.
%
This leads to observations that form the rest of this section.


\subsection{Slowest Particle}


Table~\ref{tab:long_particle} shows data collected from the slowest particle for each of the configurations involving 128 ranks and $2000$ steps.
%
The table is organized according to Equation~\ref{model:eq2}. 
%
There are several interesting trends that require more investigation.
%
First, advection and communication and wait time take a significant
amount of time.
%
While this is not unexpected, the magnitudes are surprising.
%
This is explored in Section~\ref{sec:adv_and_wait}.
%
%
Second, the variation in alive time varies considerably.
%
This is explored in Section~\ref{sec:variation}.
%
Third, ``end overhead'' (EO) is taking a significant portion of the
overall execution time.
%
This is explored in Section~\ref{sec:eo}.
%

\clearpage

\begin{figure*}[ht]
\centering
\includegraphics[width=180mm]{./figs/ParticleLongExec/particle_gantt_five_datasets_red_wait.pdf}
\caption{Gantt charts of the particle with long execution time for evaluated data sets when there are $128$ blocks and $2000$ advection steps. The pink color represents wait and communication time. Other colored bars represent the advection time. In particular, advection in different blocks is represented by one color chosen from the viridis color map. The white colored slot during the particle execution between the pink colored bar and other colored bars represents other overhead.}
\label{fig:particle_long_exec}
\end{figure*}


\subsection{Advection and Wait Times}
\label{sec:adv_and_wait}

Figure~\ref{fig:particle_long_exec} shows Gantt charts of an individual particle for a workload of 128 blocks and 2000 advection steps for all datasets.
%The bars in the chart are colored by the rank ID where the particle resides. The width of the bar indicates how long the particle is on a given rank for advection. The spaces between each bar indicate that a particle is waiting to be processed (e.g., being communicated, waiting in the queue for processing, etc). 
%
Consider the CloverLeaf3D Gantt Chart,
which shows a particle bouncing between a few MPI ranks (colored purple, dark blue,
and dark green) before ultimately bouncing back and forth between a ``green''
MPI rank and a ``yellow'' MPI rank.
%
Each time it travels to the ``green'' MPI rank, there is a considerable delay
before it can be processed.
%
Table~\ref{tab:long_particle} shows that this particle takes 229.6s to
complete, of which 45.92s is spent doing advection (20\%) and
159.34s is spent waiting to be processed.
%
Both numbers are affected by load on the MPI rank.
%
For the delays before before processing on the green rank, the issue is that
the green rank is working on a large batch of particles when the slowest
particle arrives.
%
It therefore waits in a queue.
%
This is the biggest factor in overall execution time.
%
Next, when it is time to do advection, the slowest particle is processed in
a large batch of particles.
%
It likely only takes microseconds to carry out the slowest particle's advection
steps, but the time to carry out the rest of the particles in the batch
is significant.
%
This is effectively a second kind of wait --- waiting for particles within
the batch to finish.
%
In all, the biggest factor in slow performance is that a given MPI rank needs
to process a large number of particles at one time.
%
This factor is revisited in Section~\ref{sec:opportunities}, which explores
performance from an MPI rank-based perspective.

\hank{Do we have something about motorcycle gang size?  Also, how long would
it take to do the steps for a single particle on a single core?}

\clearpage

\begin{figure}[ht]
\centering
\includegraphics[height=50mm]{./figs/ParticleLongExec/SupernovaChangeRecvs.pdf}
\caption{The accumulated time for different stages of long running time of Supernova data set when there are $128$ blocks and $2000$ steps.}
\label{fig:chage_recv}
\end{figure}

\hank{here is some clearly useful and relevant text on big batch sizes that I did not integrate well. I think this can help tell the story of different batch sizes and how we are screwed no matter what we do.}

\dave{Remove the packet-text. Also address the overhead above as setup for talking about the particle gantt charts.}
Another observation stemming from Figure~\ref{fig:particle_long_exec} is the existence of wait time for long running particles. Each time when a tracing particle moves to a new block, it introduces extra wait time and overhead, such as getting particles and small advection steps closing to boundary. The length of accumulated wait time is influenced by configurations of asynchronous MPI protocol used in the study. The associated protocol decompose message into several small packets with fixed length, and the number of alive \texttt{MPI\_Irecv} (termed by ``receivers'' in this study) remains constant during the particle execution. The particles stored in message will be extracted and advected only when all packets are received by a receiver.

Figure~\ref{fig:chage_recv} illustrates accumulated wait time, advection time, and other overhead on average (three runs) for a long running particle.  The Supernova data set is adopted in this experiment, and the number of receivers changes from $64$ to $1024$. There is a tradeoff between accumulated wait time, accumulated advection time, and other overhead. When we use a large number of receivers, such as $1024$, the message will be received within fewer iterations in receivers, resulting in a reduction of accumulated wait time. However, the size of the particle group and the targeted particle increases, leading to more accumulated advection time and other overhead.



\clearpage


\begin{figure*}[ht]
\centering
\includegraphics[width=180mm]{./figs/ParticleTermination/particles_all_dots_statistics_all.png}
% There are some issues in prev gang size, we only measure one previous gang, there are actually multiple gangs
\caption{Visualization of statistics when particle terminated with $128$ ranks and $2000$ advection steps. In particular, Subfigure (a.1)-(a.5) shows alive time of sampled particles (sample rate is $100$) in ascending order for evaluated data sets. Subfigure (b.1)-(b.5) shows accumulated group size of particles sorting by their alive time. Subfigure (c.1)-(c.5) shows accumulated previous group size of particles sorting by their alive time. Subfigure (d.1)-(d.5) shows number of traversed blocks for particles sorting by their alive time.}
\label{fig:particle_statistics_details}
\end{figure*}


% Maybe considering removing this scatter plot 
\begin{figure*}[ht]
\centering
\includegraphics[width=180mm]{./figs/ParticleTermination/particles_all_dots_all.png}
\caption{Scatter plot of particle when they are terminated. There are $128$ ranks and $2000$ advection steps. The $x$ axis represents the ratio of particle active time to the particle advection execution time. The $y$ axis represents the number of traveled blocks for each particle. The denser colored regions represents more number of terminated particles. The larger circle corresponds to a larger accumulated group size when particle terminates. \dave{Different way to plot the gang size?}}
\label{fig:particle_scatter}
\end{figure*}

\begin{figure*}[ht]
\centering
\includegraphics[width=180mm]{./figs/ParticleTermination/particles_bars_all.pdf}
\caption{The colored bars represent the number of terminated particles (labeled on the left $y$ axis) when using $128$ ranks and $2000$ advection steps. Different color represents different termination reasons. 
The orange curve represents the number of active particles (labeled on the right $y$ axis) within a specific time slot during the particle execution .}
\label{fig:particle_num}
\end{figure*}

\subsection{Variation in Alive Time}
\label{sec:variation}

Alive time is the sum of all of the factors in Equation~\ref{model:eq2}. 
%
Further, the dominant terms of advection and waiting were 
discussed in the last section.
%
This section considers why the overall alive time varies so much, ranging from
6.5s to 229.6s even though the proportion spent in the individual terms
of the model do not vary nearly as much.
%
One crucial aspect is the load on a given MPI rank.
(\hank{we need more statistics on this!} \matt{what about measuring the total time of longest particle, but without any other particles?} -- \dave{Matt, This is a very interesting idea... and easy to run.})
%
Another aspect is particles terminating early, whether
because they exit the domain, because they enter a sink, or
they enter a zero-velocity location.
%
This section considers early termination, which has the further
benefit of reducing load on a given MPI rank.



\if
\dave{Should this go before the particle gantt charts? Need to tie these results to Eq 2.}
The previous subsection discusses the execution path of long running particles, while the current subsection presents statistics for all particles. 
During each run, data are collected for each particle. These include the time when a particle terminates, the number of blocks traversed by the particle, and the reason the particle terminated. Reasons for termination are as follows:
\begin{itemize}
    \item Out of bounds: The particle exited the spatial bounds of the dataset.
    \item Zero velocity: The particle enters a sink.
    \item Max step: The maximum number of advection steps is achieved.
\end{itemize}
\fi

Figure~\ref{fig:particle_scatter} provides a holistic view of statistics for when particles terminate over each dataset. 
%\dave{insert comment on particle sampling.. Why not Synthetic?}
% Jay, synthetic results are added, and we also added how particles are sampled
We sample the particle with a sample rate of $200$ and scatter associated particle statistics in the figure. In particular, the X axis is the execution time, normalized to 1. The Y axis is the number of blocks traversed by a particle. The color indicates the particle termination reason. The denser color represents more particles terminated in the corresponding region, and a longer diameter of a circle point indicates a larger accumulated group size when a particle terminates.
For the Tokamak data set, the number of traversed blocks remains constant at the half stage of particle execution; the long running particles are mainly caused by the large size of the particle group. The Supernova data set indicates that both the large number of traversed blocks and group size can contribute to the long execution time. Intriguingly, particles terminating at around $60\%$ of execution time, despite sharing a similar number of traversed blocks with the particle terminating at around $100\%$ of execution time, demonstrate a smaller group size and consequently less execution time. In addition, Hydraulics and CloverLeaf3D data sets also indicate that the particles having the longest execution time are caused by a large number of traversing blocks and accumulated group size. These results are aligned with the theoretical consideration discussed in subsection~\ref{subsec:model:particle}.

%\james{The figure associated with this section is not clear. You use the term "available" and "active" interchangeably, which is somewhat confusing. The fact that the color legend should be used from the previous figure was not immediately clear, as it is a standalone figure, not a subfigure. Which y-axis went with which data was not clear. A legend would fix this (though I would not use a blue curve while also using blue bars in the same figure). }
% Jay, figure and associated descriptions are updated


\begin{table}[ht]
\begin{center}
\caption {Percentage of terminated particles with different reasons for $128$ data blocks and $2000$ advection steps.}
\label{tab:particle_exit}
\begin{tabular}{llll}
\toprule
Data sets &  Out of bounds & Zero velocity &  Max steps  \\
\midrule
Tokamak  & $2.1\%$  & $69.1\%$ & $28.8\%$  \\
\midrule
Supernova  & $82.5\%$  & $8.5\%$ & $9.0\%$  \\
\midrule
Hydraulics  & $39.6\%$  & $59.0\%$ & $1.4\%$  \\
\midrule
CloverLeaf3D  & $15.1\%$  & $41.9\%$ & $43.0\%$  \\
\midrule
Synthetic  & $26.2\%$  & $12.7\%$ & $61.1\%$  \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


\james{What is the takeaway here? The paragraph describes what we can see, but not what we learn. Short takeaway and a forward reference to the discussion if necessary}
\textcolor{red}{Jay, we added some take away information, maybe need to discuss more}
\matt{How about: since groups have a large influence on the overall time, this needs to be studied in greater depth. At the extreme, this is a ``streaming'' system that attempts to minimize the group effect in multi-core scenarios.}

Figure~\ref{fig:particle_num} further illustrates the number of terminated particles over time. The colored bar represents the number of terminated particles for each time slot, and the blue colored curve represents the number of active particles. For Tokamak, Supernova, and Hydraulics data sets, the number of active particles drops quickly at the early stage of the execution and then decreases gradually till the end of the particle advection. For CloverLeaf3D, the number of alive drops to $100,000$ particles and maintains this level throughout the course of execution.


Experiment results shown in particle-centric analysis reveals why there are different execution time for evaluated data sets with the same workload configurations. For example, there are a few green colored bars for Hydraulics in Figure~\ref{fig:particle_scatter}, which shows that most of the particles are terminated before completing all advection steps. In particular, only $1.4\%$ particles for the Hydraulics data set complete all their advection steps. Therefore, Hydraulics takes less time to complete particle advection compared with other data sets. Although the Supernova data set has $9.0\%$ particles completing all advection steps, it takes longer execution time than the Tokamak data set, which has $28.8\%$ max step particles. This is because the Supernova data set has more particles passing back between adjacent data blocks (illustrated in Figure~\ref{fig:particle_long_exec}), and these particles increase the particle advection's execution time.

\clearpage

\begin{figure}[ht]
\centering
\subfigure{
\includegraphics[height=35mm]{./figs/Astro-pingpong}
}
\hspace{5mm}
\subfigure{
\includegraphics[height=35mm]{./figs/Clover-pingpong}
}
\caption{Examples of a particle that ping pongs in the Supernova (left figure) and Cloverleaf3D (right figure) dataset. The long running particles are trapped into a vortex crossing two adjacent data blocks.}
\label{fig:example_pingpong}
\end{figure}

\subsection{End Overhead and Ping Pongs}
\label{sec:eo}

As discussed in the previous subsection,
particle can be repeatedly passed back and forth between two compute ranks. In particular, in the  Supernova and CloverLeaf3D datasets, the stage where the particle is circulating back and forth between ranks takes more than half of the total execution time.
Particles exhibiting this behaviour are shown in Figures~\ref{fig:example_pingpong} for the Supernova and CloverLeaf3D datasets. A vortex exists in each dataset that is near a block boundary that results in particle circulation between the two blocks.
We provide a more detailed analysis and explore methods to alleviate this situation later in Section~\ref{discus:pingpong}.

\hank{I am unhappy with this.  More quantification.  Also quantification of End Overhead.}
\dave{We need to discuss the small-step issue as well.}

\clearpage
\section{Results: Opportunities for Improvement}
\label{sec:opportunities}

\subsection{Rank-centric Analysis}

\label{results:rank-centric}

%\begin{figure*}[ht]
%\centering
%\includegraphics[width=\linewidth]%{./figs/summary_timings}
%\caption{Summary timings.}
%\label{fig:summary_times}
%\end{figure*}


\begin{figure*}[ht]
\centering
\includegraphics[width=181mm]{./figs/ScaleEfficiency/all_exec_eff_time.pdf}
\caption{The first row of figures show execution time of the particle advection filter for all evaluated datasets with different number of ranks. The log scale (the base value is 2) is adopted for both $x$ and $y$ axis. \hank{Y-axis should be log scale, but it should have the values pre-log, not the results of the log.} The second row of figures show weak scaling efficiency of all evaluated data sets with different number of ranks. 
%\ken{The x-axis should be labeled (\# of ranks).}
%\ken{The y axis for efficiency should all be scaled from 0 to 1.}
% Jay, the x label and y axis is updated
}
\label{fig:results:scale}
\end{figure*}


Figure~\ref{fig:results:scale} shows the total execution time for a weak scaling run on each of the five data sets. As described above, we maintain a fixed seed count of $5000$ for each data block, and assignment of one block per rank. As such, the number of ranks and the number of blocks is the same. The number of steps varies between $50$ and $2000$.

The weak scaling efficiency for each experiment is shown in (a.2) to (e.2) in Figure~\ref{fig:results:scale}.
The weak scale efficiency for a run with $N$ ranks is defined as the ratio $T(N)/T(8)$. $T(8)$ is time to execute an experiment with $8$ ranks (the lowest level of concurrency) and $T(N)$ is the time to execute an experiment with $N$ ranks.
This is consistent with a unit-cost-based efficiency \cite{Moreland2015:ISC} using the 8-rank case as a base and recognizing that the problem size increases proportionally to the number of ranks.
Perfect scaling gives an efficiency value of $1$ for all $N$.
The weak scaling efficiency over all experiments significantly declines as the number of ranks increases, even for cases that are ideal for the POD algorithm (i.e. Tokamak and Synthetic).
Additionally, the efficiency drops as the number of advection steps grows and is particularly pronounced in the Supernova and CloverLeaf3D data sets.


Gantt charts provide an effective way to understand the activity of each rank over the course of the execution.
Figure~\ref{fig:results:gantt} shows Gantt charts for a workload consisting of 128 ranks and 2000 steps for each dataset.
In these figures, blue regions represent the advection time, the pink regions account for both wait time and communication time, and the white region represents other associated overhead. 
%\ken{I would call that pink, not red. Also, see my comment in the caption of Figure \ref{fig:model:rankgantt}.}
These charts provide an overview of the overall balance of work among the ranks and give insight into the overall scalability.
The Gantt charts for the Tokamak, Hydraulics, and Synthetic datasets appear to have more balanced workloads.
Conversely, the Gantt charts for Supernova and CloverLeaf3D clearly illustrate that the reason for long execution times is that a relatively small number of ranks have much more work, which results in poor efficiency.
\dave{A big part of the problem is that the particle path has to be executed in order -- the amount of parallelism is constrained.}
%In particular, the Gantt charts for Supernova and CloverLeaf3D data sets reveal the presence of ranks with a significantly longer execution time than others. These ranks with a long execution time cause the work imbalances and low weak scale efficiency. Conversely, Gantt charts from the remaining three data sets show more balanced workloads throughout the particle execution. To quantitatively assess the varying degree of each rank's involvement in particle advection processing over time, a suitable metric needs to be developed further.
\dave{Insert references back to equation 1.}








To  quantify the overall efficiency, we introduce a simple metric called \emph{rank participation} to illustrate the overall performance of the algorithm over the course of execution.
Rank participation is defined as the fraction of ranks actively doing work.
Specifically, if $N_T$ is the total number of ranks in the parallel job and $N_A$ is the number of ranks actively doing work, then the rank participation is $N_A/N_T$.
The rank participation can be measured instantaneously or integrated over the execution of the algorithm.
A rank participation of $1$ represents a perfectly load balanced operation whereas a small rank participation of $1/N_T$ means one rank is working while the rest remain idle.



%\begin{figure*}[ht]
%\centering
%\includegraphics[width=\linewidth]%{./figs/fusion_astro_64_gantt_RP}
%\caption{Representative Gantt chart and associated rank participation chart}
%\label{fig:summary_gantt}
%\end{figure*}

\begin{figure*}[ht]
\centering
 
%\includegraphics[width=180mm]
%{./figs/GantCharts/rank_gantt_all.png}
\caption{Gantt charts for evaluated data sets when there are $128$ ranks and $2000$ advection steps. \hank{Hank removed image so his PDF would compile.  It should not be removed permanently.  And Hank meant to add it back in so no one would see he did this -- whoops.}}
\label{fig:results:gantt} 
\end{figure*}





\begin{figure*}[ht]
\centering
\includegraphics[width=180mm]{./figs/Participation/rank_participation_all.pdf}
\caption{Participation rates when there are $128$ ranks and $2000$ advection steps for evaluated data sets.}
\label{fig:scale}
\label{fig:results:pr}
\end{figure*}

%\dave{participation rate images: add charts with more ranks/steps. Can normalize the runtime so that multiple runs can be put in 1 plot.}
% Jay: the exeuction time is a little bit different for different configurations, maybe we need double check about the proper visualization results, I tested 128 blocks with 50 steps, which has similar trend with current results. 

Figure~\ref{fig:results:pr} shows the rank participation values for the same runs shown in Figure~\ref{fig:results:gantt} ($128$ blocks and $2000$ advection steps).
%\ken{It just occured to me that the phrase ``rank participation rate'' is used several times. Is rank participation really a rate? A rate generally compares things of different units, which is not the case here. I suggest removing rate and just say ``rank participation''.}
% Jay: we updated it into rank participation and aggregated rank participation
The rank participation curve provides a straightforward view of the number of ranks actively engaged as the algorithm progresses. We note that a rank is marked as participating when it is performing any of the following tasks: $A$, $BO$, $EO$ and $C$ from Equation~\ref{model:eq1}. And conversely, a rank is marked as not participating when it is idle (task $W$ from Equation~\ref{model:eq1}.)
The participation rate charts highlight the problems with efficiency for the Supernova and CloverLeaf3D datasets as there is a dramatic drop in participation at the outset of the execution.
The Tokamak and Synethetic datasets exhibit relatively consistent and steady participation rates over the course the execution while the Hydraulics dataset lies somewhere in the middle.

We further compute the \emph{aggregated rank participation} over the course of a run by integrating the participation rank curve (the area under the rank participation curve) across a normalized time axis. If all ranks were engaged across the entirety of the run, the aggregated participation rate would be $1.0$. 
The aggregated rank participation values are shown in Figure~\ref{fig:summary_RP} for all of the experiments examined in our study. All of the runs for a given dataset are shown as a subplot.
The curves in each subplot track the aggregated rank participation for a run at a given level of parallelism as a function of the number of advection steps.
As an example, the purple line in the Tokamak subplot shows the aggregated rank participation running on $128$ ranks and advection steps of 50, 100, 500, 1000, and 2000.
Plotting these metrics provides insight into the scalability of the algorithm across different datasets and workloads. 
Specifically, Tokamak and Synthetic data have high average rank participation values, whereas Supernova and CloverLeaf3D exhibit lower participation values when the number of ranks increases from $8$ to $128$. The average participation rates are more sensitive to the number of ranks for Supernova and CloverLeaf3D data sets compared to other datasets. 
%\dave{A lot more graphs are available for participation rate. I think more would explain what is going on. Participation rate and weak scaling are related so these need to be discussed together.}
% Jay: we added weak scaling efficiency to further explain the results

\begin{figure*}[ht]
\centering

\includegraphics[width=180mm]{./figs/Participation/rank_participation_gather_all.pdf}
\caption{Aggregated participation rates across all evaluated datasets.  
%\dave{X axis is Total number of advection steps, OR, put a dot on each experiment.} %\dave{change plot axes title to aggregated.}
}
% Jay, x y axes are updated and the dot is added into the figure
\label{fig:summary_RP}
\end{figure*}



\if 0
\subsection{Particle-centric Analysis}
\label{subsec:pstatus}
Rank-centric analysis provides a broad perspective of algorithm efficiency.
Evaluation results shown above in Section~\ref{results:rank-centric} reveal the degrees of workload imbalance across evaluated data sets and workloads.
It lacks, however, the ability to provide a clear insight into the barriers to scalability.
To probe more deeply into scalability issues we explore the model analysis in section~\ref{subsec:model:particle} and study the performance from a particle-centric perspective. 
\fi



%\subsubsection{Oldest particle analysis}
\if 0
\subsubsection{Long running particle analysis}

Algorithm execution time is determined by the particle with the maximum execution time (Equation~\ref{model:eq2}). 
Because of this, investigating particles with long execution time can offers insights into algorithm performance.
Collecting the data from Equation~\ref{model:eq2} for each particle would introduce significant overheads. To avoid this problem we collect data on a representative particle with a long execution time.
Determining a representative particle is straightforward. When the algorithm is run we record the ID of the last particle that terminates. We then re-run the algorithm and collect data only on the particle with that specified ID.
In practice, when using asynchronous communication, the particle with the longest execution time is not always the same, but the execution times are similar enough that it provides an accurate representation of the longest running particle.



%\dave{Do we want to show and discuss this table?}
The data in Table~\ref{tab:long_particle} shows data collected from the long running particle for the 128 rank cases of $2000$ steps over each dataset.
The values for each variable in Equation~\ref{model:eq2} are shown as a percentage of the total time for the particle. 
\ken{I'm reading this paper out of order, so I might have just missed it, but is it described how the terms of Equation \ref{model:eq2} are measured? I expect $A$ is everything in the advection loop, and $BO$ and $EO$ are the things before and after this loop, respectively. How do you differentiate when a particle is communicating and when it is waiting?}
\dave{I think we need some sort of graphic that describes what we are timing. Perhaps a block or state diagram.}
\james{This large table only gets one small paragraph of explanation. Further, there doesn't seem to be a takeaway here. What am I supposed to understand from this analysis? Just emphasizing that your model has different components? Maybe a forward reference to where you explain the differences in advection vs wait time for different step sizes? Then, the next few graphs only talk to the 2000 step case. Is the 1000 step important here, if so, that should be a finding in the text. Next, a refresher on the equation should be in the table or the text, that was many sections ago. Lastly, without expanding the explanation quite a bit, I think the other graphics are more compelling, so this could be skipped.}

%\input{sections/percentage_table}

\fi



%\james{This figure would be much more compelling at full page width. Also, the zoomed in view is not showing anymore.}
% Jay: the Figure9 is updated to full page width
%\dave{We need to provide a clear explanation of what we are recording. syncronized time stamps are set on a particle whenver it goes into the worklet.Advect(). Explain what is going on in the white space.}
%It is worth noting that these Gantt charts are rendered with limited precision. Very thin bars get inflated to a minimum (pixel) width.
%For instance, in Figure~\ref{fig:particle_long_exec:b}, a zoomed-in view of the Gantt chart for the Hydraulics dataset offers a more detailed perspective.


%\subsection{Reasons for poor performance}


%\begin{itemize}
%    \item Participation rates.
%    \begin{itemize}
%        \item Story: problem exists, gets worse at scale for many data-sets.
%        \item Gantt charts for 2 cases and participation plot
%        \item Table with percentages
%        \item summary chart: Astro: x= numsteps, y= participation. show lines for 8,16,32,64,128,... (similar to figure 3)
%        \item insert discussion from slides on what to discuss here.
%    \end{itemize}
%    \item why the participation is so bad. Item 1 is ping pong.
%    \item Ping pong
%    \begin{itemize}
%        \item show traces of codes, discuss paterns
%        \item rank and particle gantt charts
%        \item Astro has LOTS of ping pong particles. (rank particle , step charts)
%        \item how it appears / disappears with num blocks. Show gantt chart at 8 ranks, 16, compared to 128. Consider the other charts if needed. (final rank)
%    \end{itemize}
%\end{itemize}


%Two problems exist. participation, ping pong.
%ping pong and number of blocks. astro vs. fusion/synthetic

%Discuss the magnitude. how bad it hurts.


==> sections/EGPGVreviews.tex <==
\section{Reviews}


\begin{itemize}
    \item \textbf{R4- Summary Review}
    \begin{itemize}
        \item Finding that seed distribution impacts performance is obvious
    \item test cases too narrow to draw conclusions
    \end{itemize}
    
    \item {R1 - reject}
    \begin{itemize}
        \item Lack of contribution. Authors overstate their findings.
        \item No surprising results.
        \item The magnitude of the numbers are not obvious but not surprising
        \item What should we do with this information? What is the followup research? What changes should be made?
    \end{itemize}

    \item {R2 - Borderline}
    \begin{itemize}
        \item Positive: Findings of sensitivity to inputs
        \item results are not that surprising, but the magnitude of badness is surprising.
        \item Location of the boxes need to be explored and impact on participation need to be better explored (discussion on Fig 2 and 3)
        \item Interesting result for the community but needs some more detailed analysis.
        \item good suggestions re: execution times and how much this matters at small scale.
    \end{itemize}    

    \item {R3- argue for accepting}
    \begin{itemize}
        \item Contributions of the paper are good....
        \item plot clarity on x-axes in figures 3,4
    \end{itemize}    
\end{itemize}


\subsection{Summary Review}
I see the basic idea of good experiments for comparing used algorithms as valuable, but the contribution of this publication is rather limited as it only describes two implementations and is tested on a single computer without changing parameters there. So no general conclusion may be drawn from the work.

The outcome that the speedup depends on the initial distribution of particles is nothing impressive. The quality would improve if the dependency could be formulated in a way that help to speed up the algorithms.

Summary Recommendation:
Probably reject: The reviewers argue for rejection.
Summary Review Text:
All reviewers agree that the contribution of the paper is limited and the results rather obvious.
A larger study with a broader set of dataset may be beneficial for the community, but the publication is not there, yet.



\subsection{R4 - coordinator}

Reviewer 4 (coordinator)
Overall Rating:
Borderline: The strengths and weaknesses balance for this paper.

Expertise: Knowledgeable

Summary Review:
The authors perform timing tests on two spatial distributions of the algorithm workload for particle advection.

Contribution:
The contribution consists of experiments with comparing two techniques by measuring the performance of particle advection.
The contribution is valuable but rather limited to this special algorithm and I am not sure whether general assumptions can be drawn from those experiments.

Clarity of Exposition:
The exposition is clear.

Technical Soundness:
The procedure is technically sound, but rather limited to the special case as described in the contribution section of this review.

Quality of References:
Important references are present.
Reproducibility:
The paper could be reproduced as is.
Evaluation:

Explanation of Recommendation [Regular Submission]
I see the basic idea of good experiments for comparing used algorithms as valuable, but the contribution of this publication is rather limited as it only describes two implementations and is tested on a single computer without changing parameters there. So no general conclusion may be drawn from the work.

The outcome that the speedup depends on the initial distribution of particles is nothing impressive. The quality would improve if the dependency could be formulated in a way that help to speed up the algorithms.

Summary Recommendation:
Probably reject: The reviewers argue for rejection.
Summary Review Text:
All reviewers agree that the contribution of the paper is limited and the results rather obvious.
A larger study with a broader set of dataset may be beneficial for the community, but the publication is not there, yet.


\subsection{R1}
Reviewer 1 (committee member)
Overall Rating [Regular Submission]
Probably reject: I would argue for rejecting this paper.
Expertise [Regular Submission]
Expert
Summary [Regular Submission]
In this paper, the authors compare the effects of different seed strategies for particles when parallelizing particle advection with the POD method.
Contribution [Regular Submission]
Lack of contribution is my crucial criticism of the submission. See below.
Clarity of Exposition [Regular Submission]
The paper is written well and easy to read.
Technical Soundness [Regular Submission]
Within its limited scope the paper is sound.
Quality of References [Regular Submission]
For a short paper, the references are adequate.
Reproducibility [Regular Submission]
It should be straight forward to reproduce the results.
Evaluation [Regular Submission]
I think the authors overstate the importance of their findings.
Explanation of Recommendation [Regular Submission]
Lack of contribution is my crucial criticism of the submission. I have a hard time understanding the contribution of the paper. Mostly, the results make sense, but nothing reported in the paper is surprising, and the results appear trivial to me and are very much what I would expect. Of course, the exact figures (utilization percentages) are not obvious, but the order of the numbers will hardly surprise people familiar with the topic. So my question is simply: Who will benefit from this result? What follow-up research will be possible? What systematic changes in existing approaches can be made to the existing software/hardware based on these findings? So far, my answer would be "none" to all of the questions above.

Besides my big conceptual concern raised above, I'm surprised that the authors used such small datasets. How can you be sure that your results remain valid with real datasets?

There are a few minor issues that can be fixed easily. The definition of the rank participation is a bit inconsistent. In the introduction it is defined as a quotient, explicitly saying that range is between 1/Nt and 1 but the rest of the paper uses percentages. This is no big deal but I would constantly use percentages.
"Table 1 shows the average participate rate by data ... " should be "Table 1 shows the average participation rate by data..."


\subsection{R2}
Reviewer 2 (committee member)
Overall Rating [Regular Submission]
Borderline: The strengths and weaknesses balance for this paper.
Expertise [Regular Submission]
Knowledgeable
Summary [Regular Submission]
This article provides benchmarks of PoD approaches for particle advection algorithms, focusing on the CPU participation in a distributed environment and how it evolves regarding several parameters. The focus is set on the inherent algorithmic properties and thus the authors tries to remove most external problems, arising due to network infrastructure, jobs concurrency or data movement to the GPU.
Contribution [Regular Submission]
Thanks to theirs benchmarks, the authors have found that PoD approaches are sensitive to the initial seed distribution with a spectacular drop of performance for smaller seed distribution, especially for data set where these particles converge. Even is this conclusion goes into what some could expect regarding these kind of algorithms, the effect may be more impactful than initially though and is quantitatively measured here.
Clarity of Exposition [Regular Submission]
The article is well written as well as well illustrated. Contribution are clearly stated.
As we will see later, some parameters are chosen but not necessarily completely justified.
There is a minor suggestion regarding on confusing time operation that will be given in the last paragraph of this review.
Technical Soundness [Regular Submission]
The article is technically sound. OK.
Quality of References [Regular Submission]
Citation for important terms are present, previous work discussed. OK.
Reproducibility [Regular Submission]
The amount of details given is sound, but there some missing information that would be required for reproducibility. Without going up to the Guix like reproducibility, the source of the benchmark would be a great addition to allow one to have a look at some specific details. For example, in the case of the Box 50 / 25 / 10 / 5 (which drives the conclusion), it is not clearly stated where this boxes are initially located. From the Figure 2, it would seems the Box 10 is in a single rang initially as we see the workload going from rank to rank almost sequentially, but in Figure 3, the initial workload is often more that one rank even for Box 50 / 25 and even in some cases for 10. This is an important point.
Evaluation [Regular Submission]
Previous work is discussed, no comparison with other existing analogous benchmark.
Explanation of Recommendation [Regular Submission]
As already stated, I think the conclusion of this article is interesting for the community as it emphasize where looking for improvement would be relevant for these kind of widely used algorithm. However there are several points that would need to be addressed in my opinion:

* Execution times are really small. At this scales, lots of small things may impact the result time (context switch, process launching, ... ) This is of course mitigated by the large averaging of several simulations, but sub-second benchmark may not be as reliable. Could we have some discussion about the internal variation of execution times ? The standard deviation and min / max time for example, that would help decide if those timing are relevant.
* As stated earlier, the smaller box play an important role in the conclusion, unfortunately the box disposition is not clearly stated so it is not clear how many ranks have jobs in the initial steps. This may not be so impactful after a large number of time-step anyway.
* I like how the datasets seems to lead to various behavior regarding the particles, could we have a small metrics on the convergence / divergence of the particles ?

Minor remarks:

It is stated that box larger than $64 ^ 3$ would harm efficiency, could we have a short word on why ?

On the result part, we have a 80.1% which becomes 0.81 (typo)
On this part, we have some confusing computation. If there is a 0.80 efficiency, a 100% efficient algorithm would be 100 / 80 = 1.25 times faster. I find the current explanation a bit confusing here.

\subsection{R3}

Reviewer 3 (committee member)
Overall Rating [Regular Submission]
Probably accept: I would argue for accepting this paper.
Expertise [Regular Submission]
Knowledgeable
Summary [Regular Submission]
The paper presents a performance study of the parallelize over data particle advection approach, evaluating the efficiency of this widely used technique. The study is performed on a number of different data sets, different initial particle seed configurations, and advection durations, providing a detailed evaluation of the method’s performance. The resulting load imbalance is reported for these different configurations, providing motivation for use and research of other methods. While the evaluation is run on only 8 cores this is fine, as increasing the core count/distributed run size would only increase load imbalance issues further.
Contribution [Regular Submission]
The contribution of the paper is the detailed performance evaluation of a known and widely used algorithm. This contribution of a detailed study/performance results seems fine for a short paper, providing a data point for other research.
Clarity of Exposition [Regular Submission]
The paper is well written
Technical Soundness [Regular Submission]
The implementation and evaluation seem to be sound.
Quality of References [Regular Submission]
The references seem fine for a short paper.
Reproducibility [Regular Submission]
The approach is well known and evaluation well described such that it should be easy to reproduce the study.
Evaluation [Regular Submission]
The evaluation is thorough and is the main contribution of the paper. A large number of data sets, seed configurations, and advection durations are evaluated, with detailed results reported for each configuration to inform other researchers.

To make the advection over time results plots easier to read it may be worthwhile to not plot the timestamp value as a numerical value along the x-axis in Figures 3 \& 4, as this has the effect of squishing the low advection time results together and making them hard to read. These time values could instead be plotted as discrete “labels” to space them evenly along the x axis.
Explanation of Recommendation [Regular Submission]
The detailed performance study of a widely used algorithm contributed by this short paper is a useful contribution to the literature to provide a data point for other researchers, and is sufficient for a short paper. Thus, I lean to accept.

Return to submission and reviews

==> sections/NOTES.tex <==
1. no participation trophy for you
2. ping effect

here's an effect, it's real. magnitude of it all.

Contribution: wer're pointing out hte problem and its magnitude.
here are some potential solutions.
Ken's things.
1- identify when ping pong happens. kill the particle. could be hard with complex loops. Fishtank example
2- block duplication to bring in the extra block to address ping pongs. (dynamic approach)
3- make really wide ghost zones.
4- pre-process to identify the vorticity and find where these issues might occur. (static approach)

if we do an in situ FTLE, we do what's in this particle.
in situ vs. post hoc considerations: terminate loop in situ might be the way to go.

TODO:
Jay finds the IDs for the long particles. Do the runs.
run the ping-pong locations.

synthetic 64 ranks, 1 particle. many hops, less hops. look at time.
100 particles. motoctocle gang.
Syn: 64 blocks, particles: 1,10,1000, steps=4000, Box='G' *DONE*
Resample 64 onto 2x2x16 (less hops) Box= 'H' *TODO*

long particle on astro: run at 8, 16, 32, 64, 128, 256.
Jobs submitted

Hank: Intro, discussion.
Jay: partticle gant chats.
gannt charts -- all runs.



Waiting flavor 1: i'm in a big gang
Waiting flavor 2: a big gang is already there before me

the more ping pongs you have the more opportunities for flavor 2.

==> sections/acknowledgment.tex <==
\section*{Acknowledgment}

==> sections/overview-EGPGV.tex <==
\section{Experimental Overview}
Our experiments are designed to explore rank participation using a diverse set of data sets, seeding strategies,
and durations. Although our study does not cover all possible factors that affect particle advection
performance, we choose to vary these particular factors to explore the efficiency of the algorithm over
a set of idealized workloads.

All data sets are divided into 8 blocks, and each block is a $64^3$ uniform grid except for Clover, which is
$128\times{}128\times{}256$ per block. All experiments are performed on a single 8 core workstation to minimize the effects of network traffic and node variability.
This configuration represents a reasonable best possible case;
increasing the data set size and the number of MPI tasks will only result in worse efficiency. Additionally, the configuration's simplicity helps us reason about the results. We used five data sets:
%\dave{8 blocks, 8 MPI tasks and the reasons for doing it.}
%\dave{This is a reasonable ceiling, will only get worse.  
%***
%This is a hard problem, simplicity helps us to understand what is going on.
%Simple, easy to understand.}
\begin{itemize}
  \item \textbf{Tokamak}: a torus-shaped vector field from a magnetically confined fusion simulation. See Figure~\ref{fig:fusion}.
  \item \textbf{Supernova}: a vector field derived from the magnetic field during a supernova. See Figure~\ref{fig:astro}.
  \item \textbf{Hydraulics}: a thermal hydraulics simulation of a box with two inlets and one outlet. See Figure~\ref{fig:fishtank}.
  \item \textbf{CloverLeaf3D}: a hydrodynamics simulation of directional energy confined in a box. See Figure~\ref{fig:cloverleaf}.
  \item \textbf{Synthetic}: a perfectly cylindrical flow around a central axis. See Figure~\ref{fig:syn}.
\end{itemize}
The study uses 20,000 seeds and seven different seed placement strategies, each with different initial load balancing characteristics:
\begin{itemize}
    \item \textbf{Whole Box}: seeding the entire volume.
    \item \textbf{Box 50/25/10/5}: seeding particles in 50\%, 25\%, 10\%, and 5\% of the spatial dimensions, e.g., Box 50 creates a volume using 50\% of each dimension ($.5^3$) resulting in a volume $0.125$ of the original size.
    \item \textbf{Line}: placing seeds on a line (common for a stream surface).
    \item \textbf{Plane}: placing seeds on plane (common for a Poincar\'{e} plot).
\end{itemize}

For particle duration (i.e., the maximum number of steps for each particle), we choose 7 different values: 10, 50, 100, 1000, 2000, and 4000.
We run the cross product of data sets (5), seeding strategies (7), and durations (7), for a total of 245 experiments.
We run each experiment 20 times and average the results. 
%\dave{do we need to mention the averaging??}
For software, we use the particle advection implementation in VTK-m~\cite{Pugmire2018} with
the serial device adapter (i.e., each MPI process uses a single core) to eliminate shared-memory architectural differences.
%\dave{TODO: Add the B0, B1, B2, L, P imges in the supplemental. Link to the data sets. Link to repo.}

%\begin{itemize}
%    \item Datasets: fusion, fishtank, astro, clover, syn (text below from previous papers). Each dataset has 8 blocks.
%    \item duration: 10,50,100,500,1000,2000, 4000
%    \item seeding volumes: Full, .5, .25. .10, .05.  Not sure how best to describe this, but for the .5, the box was of dimensions: .5X x .5Y x .5Z where X, Y, Z are the lenghts of each axis of the entire dataset.
%    \item Ran experiments on multi-core workstation, 8 ranks.  Wanted to minimize the effects of a cluster and network contention.  MPI on a single node gives you the BEST case scenario for communication.  Serial adapter on VTK-m for simplicity.
%\end{itemize}

%The text below is from the SC09 paper.


%Astrophysics / Supernova Simulation. For the astrophysics case study, we create streamlines in the magnetic
%field surrounding a solar core collapse resulting in a supernova. See Figure 1. The vector field used is derived from
%the magnetic field computed by a GenASiS simulation [8], a
%multi-physics code being developed for the simulation of astrophysical systems involving nuclear matter [5]. GenASiS
%computes the magnetic field at each cell face. For the purposes of this scaling study, a cell-centered vector is created
%by differencing the values at faces in the X, Y and Z directions. Node-centered vectors are generated by averaging
%adjacent cells to each node. We then resample these vectors
%onto a grid of various sizes to measure performance of the
%streamline generation algorithms. For the purpose of this
%scaling study, we sampled the magnetic field onto 512 blocks
%with 1 million cells per block. Streamlines performance is
%studied for both sparse and dense seed points sets



%Tokamak / Magnetically Confined Fusion. The second
%dataset we consider here results from a simulation of magnetically confined fusion in a tokamak device. The simulation was performed using the NIMROD code [20]. This
%dataset has the unusual property that most streamlines are
%approximately closed and traverse the torus-shaped vector
%field domain repeatedly (see Figure 2). However, there are
%also streamlines that exhibit chaotic behavior and traverse
%the entire domain as integration time approaches infinity.
%This is of interest to the material presented here as highly
%localized streamlines can diverge strongly over time.



%Thermal Hydraulics. Figure 3 illustrates streamlines in a
%thermal hydraulics simulation. Here, twin inlets pump water
%into a box, with a temperature difference between the water
%inserted by each inlet; eventually the water exits through
%an outlet. The mixing behavior and the temperature of the
%water at the outlet are of interest. Non-optimal mixing can
%be caused by long-lived recirculation zones that effectively
%isolate certain regions of the domain from heat exchange.
%The time-varying simulation was performed using the
%Nek5000 code[9] on a regular grid of twenty-three million
%elements.

==> sections/participation_table.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[htb]
\begin{center}
\caption {Rank Participation averages for all data sets and seeding volumes. The entry for a data set $D$ and a seeding placement $V$ contains the average rank participation over all particle durations. Averages over all seeding placements for each data set are given in the last column. Averages over all data sets for each seeding placement are given in the bottom row. The entry in the bottom right contains the overall average over all data sets and seed placements.}
\label{table:allAvgs}


\begin{tabular}{l|lllll|ll|l}
\toprule
\textbf{\backslashbox{Data set}{Seed Placement }} & \textbf{Whole Box} & \textbf{Box 50} & \textbf{Box 25} & \textbf{Box 10} & \textbf{Box 5} & \textbf{Line} & \textbf{Plane} & \textbf{Data Set Average} \\ \midrule
Tokamak              & 83.5\% & 79.0\% & 23.9\% & 24.1\% & 17.6\% & 32.0\% & 40.7\% & 43.0\% \\
Supernova            & 61.4\% & 62.6\% & 56.2\% & 63.0\% & 27.8\% & 32.4\% & 48.2\% & 50.2\% \\
Hydraulics           & 69.5\% & 39.0\% & 34.1\% & 18.2\% & 14.3\% & 22.6\% & 46.4\% & 34.9\% \\
CloverLeaf3D         & 54.7\% & 39.1\% & 30.5\% & 18.8\% & 26.8\% & 19.4\% & 32.7\% & 31.7\% \\
Synthetic            & 92.4\% & 90.0\% & 17.0\% & 14.8\% & 18.4\% & 75.8\% & 41.1\% & 49.9\% \\ \midrule
\textbf{Seed Placement Average} & 72.3\% & 62.0\% & 32.3\% & 27.8\% & 21.0\% & 36.4\% & 41.8\% & 41.9\% \\ \bottomrule
\end{tabular}


\end{center}
\end{table*}



\if 0

\begin{table*}[htb]
\begin{center}
\caption {Rank Participation averages.}
\label{table:allAvgs}
\begin{tabular}{@{}lllllllll@{}}
\toprule
\textbf{Dataset} &
  \textbf{Whole Box} &
  \textbf{Box 50} &
  \textbf{Box 25} &
  \textbf{Box 10} &
  \textbf{Box 5} &
  \textbf{Line} &
  \textbf{Plane} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Dataset Avg\\  (no L,P)\end{tabular}} \\ \midrule
\multicolumn{1}{l|}{Tokamak}      & 0.835 & .790 & .239 & .241 & .176 & .320 & \multicolumn{1}{l|}{.407} & .456 \\
\multicolumn{1}{l|}{Supernova}    & 0.614 & .626 & .562 & .630 & .278 & .324 & \multicolumn{1}{l|}{.482} & .542 \\
\multicolumn{1}{l|}{Hydraulics}   & 0.695 & .390 & .341 & .182 & .143 & .226 & \multicolumn{1}{l|}{.464} & .350 \\
\multicolumn{1}{l|}{CloverLeaf3D} & 0.547 & .391 & .305 & .188 & .268 & .194 & \multicolumn{1}{l|}{.327} & .340 \\
\multicolumn{1}{l|}{Synthetic}    & 0.924 & .900 & .170 & .148 & .184 & .758 & \multicolumn{1}{l|}{.411} & .465 \\ \midrule
\multicolumn{1}{l|}{Box Avg}      & .723  & .620 & .323 & .278 & .210 & .364 & \multicolumn{1}{l|}{.418} & .419 \\ \bottomrule

\end{tabular}

\end{center}
\end{table*}

\fi


==> sections/results-EGPGV.tex <==
\section{Results-EGPGV}

\begin{figure*}[ht]
\centering
%\subfigure[Gantt chart for efficient execution]{
%\label{fig:gant:fusion}  \includegraphics[width=75mm]{./figs/GantCharts/fusion_gant}}
%\subfigure[Participation rate for efficient execution]{\label{fig:RP:fusion}  \includegraphics[width=75mm]{./figs/RPCharts/fusion_rp}}

%\includegraphics[height=25mm]{./figs/GantCharts/fusion_gant}
%\includegraphics[height=25mm]{./figs/RPCharts/fusion_rp}

%\subfigure[Gantt chart for inefficient execution]{\label{fig:gant:fusion-bad}  \includegraphics[width=75mm]{./figs/GantCharts/fusion_gant-bad}}
%\subfigure[Participation rate for inefficient execution]{\label{fig:rp:fusion-bad}  \includegraphics[width=75mm]{./figs/RPCharts/fusion_rp-bad}}

%\includegraphics[height=25mm]{./figs/GantCharts/fusion_gant-bad}
%\includegraphics[height=25mm]{./figs/RPCharts/fusion_rp-bad}

\includegraphics[height=68mm]{./figs/Gant_RP_Charts}
\caption{Gantt charts (left) and participation rates (right) for two experiments on the
Tokamak data set.  The top row shows an experiment with Whole Box seeding for 10 advection steps that is doing productive work 80.1\% of the time and is idle 19.1\% \ken{19.9\%?} of the time.
The bottom row shows an experiment with Box 10 seeding for 1000 advection steps that is working 27.4\% of the time and is idle
73.6\% of the time.}
\label{fig:gant_rp}
\end{figure*}

\input{sections/participation_table}

Figure~\ref{fig:gant_rp} reports execution time for two experiments on the
Tokamak data set.
%
%\dave{Add refs as Fig 2(c) once figures finalized.}
One experiment does productive work 80\% of the time.
It runs for 0.071s on
8 MPI tasks, meaning that it is doing 0.455s of productive work
($0.81 \times 0.071s \times 8$).
%
A different approach than POD could conceivably schedule work
and block placement so there is no idle time, i.e., productive work
is 100\%.
%
In this case, the approach 
would run in 0.056s ($0.455s / 8$), a 1.25X speedup.
%
The other experiment does productive work only 27.4\% of the time over
20.6s.
%
Following the same analysis, a different approach could conceivably
run as fast as 5.5s, a 3.7X speedup.
%
These two experiments demonstrate that the potential speedups 
going from POD to
an improved algorithm can be quite varied: small-ish (1.25X) to very large
(3.7X). 
%
%Further, this sort of analysis is used in the remainder of this section.
%
%In particular, the rank participation averages represent the integral
%of the participate rate figures (right side of Figure~\ref{fig:gant_rp}
%divided by the total execution time.


\begin{figure*}
  \centering
%    \includegraphics[width=1.0\textwidth,trim={0 11cm 0 0},clip]{figs/ResultImages}
\includegraphics[width=1.0\textwidth, trim={1mm 0 0 0},clip]{figs/Box_Dataset_Result}
  \caption{Rank participation percentages for the five data sets and five box-based seed placement. The horizonal axis in each plot is the maximum number of steps for each particle and the vertical axis is the rank participation percentage.
  %
The plots in the first row shows a seed placement-centric view of our experiments. Each plot for a particular box-based seed placement shows the rank participation percentage for all five data sets.
Conversely, the second row shows a data set-centric view.
Each plot shows the rank participation participation of each data set using all of the boxed-based seed placements.
  }
  \label{fig:smallMultiples}
\end{figure*}

Table~\ref{table:allAvgs} shows the average participate rate
by data set and box size.
%
The Box 5 results show that participation rate is very low, 
ranging between 14.3\% and 27.8\%. 
%\ken{The text is giving participation rates as percentages whereas the figures and tables are giving them as ratios. Is this going to be confusing to readers?}
%
Repeating the analysis from above, a different algorithm
could potentially achieve as much as a 7X speedup for these cases.
%
This potential speedup is not a surprising result for small seeding boxes,
which are known to run poorly in this configuration.
%
That said, the Whole Box results --- a configuration where POD should excel --- are more surprising.
%
These show that some results match expectations, like
the Synthetic data set with 92.4\% participation.
%
Others, however, are at a much lower rate: CloverLeaf3D is at 55\%,
Supernova is at 61\%, and Hydraulics is at 70\%.
%
For CloverLeaf3D, an improved algorithm could potentially 
be almost twice as fast for the supposed best case for POD.
%

Reading Table~\ref{table:allAvgs} left to right shows the effect of box
size.
%
Again, it is expected that POD is a poor algorithm for small boxes.
%
That said, we find it surprising how quickly the participation rate drops,
in particular from 62\% for Box 50 to 32\% for Box 25.
%
Further, the top row of Figure~\ref{fig:smallMultiples} makes the results from Table~\ref{table:allAvgs} clearer
by illustrating the spreads in performance in box size.
%
It also shows the role of duration (number of steps taken).
%
For the most part, participation rate drops as the number of steps
increases, likely because particles move toward sinks in the
data set causing some of the MPI ranks to have no remaining work.
%\ken{In some parts of the paper we use the single word `dataset' and in others we use the two words `data set'. I have no preference either way, but we should be consistent.}
%
A few configurations have increased participation rate as the
number of steps increases, 
most notably the Tokamak data set with the Box 10 configuration.
%
This is because the tokamak spins particles around in circular patterns, but 
particles get displaced vertically as they move, ultimately causing all MPI
ranks to get engaged when durations become high enough.
%
Finally, we are surprised by the spread in participation rate in the Box 50
plot.  
%
This relatively large seeding volume could result in participation rates
above 90\% (synthetic data set) and below 20\% (CloverLeaf with long
durations).

The bottom row of Figure~\ref{fig:smallMultiples} presents our experiments by data set.
%\ken{Since the prose first talks about the per-box plots (bottom row) and then the per-dataset plots (top row), it would probably be easier to follow along if the two rows in Figure \ref{fig:smallMultiples} were swapped.}
%
These plots show a surprising amount of variation with respect
to box size.
%
The Supernova data set has a fairly consistent participation rate for all
box sizes except Box 5. 
%
For Tokamak, the Whole Box and Box 50 both have relatively high participation
rate, but the remainder of the boxes are much lower.
%
Other data sets have different clustering.
%
In all, the underlying properties of the vector field appear to 
significantly affect participation rate as box size varies.
%
Although this intuitively makes sense, we are surprised by the
variation and magnitude of the effect.

\begin{figure}[ht]
\centering
%\subfigure[Line]{
%\label{fig:boxcentric:L}  \includegraphics[width=55mm]{./figs/BoxCentric/L}}
%
%\subfigure[Plane]
%{\label{fig:boxcentric:P}  \includegraphics[width=55mm]{./figs/BoxCentric/P}}
% \includegraphics[width=55mm]{./figs/BoxCentric/L}
% \includegraphics[width=55mm]{./figs/BoxCentric/P}
\includegraphics[width=\linewidth] {./figs/Line_Plane_Results}
\caption{Rank participation percentages of the Line and Plane seed placements for each data set. As in Figure~\ref{fig:smallMultiples}, the horizontal axis is the maximum number of steps for each particle and the vertical axis is the rank particpation percentage.}

\label{fig:seed-line-plane}
\end{figure}

Finally, Figure~\ref{fig:seed-line-plane} presents the special case
of seeding along a line or along a plane.
%
All three (line, plane, box) correspond to common, practical seeding configurations for
streamline plots.
%
Further, all three correspond to additional flow visualization
techiniques: box with FTLE, line with stream surfaces, and plane
with Poincar\'{e} plots.
%
Aside from the synthetic data set with seeds along a line (rake seeding),
the participation rate is not above 60\%, and often is much lower.
%
In other words, our experiments demonstrate that POD is a poor choice for these common
seeding configurations.

\if 0

%
For example, the Whole Box configuration performed very well for the
synthetic data set, which spins particles throughout the volume in a loop,
but the other 
%
But it performed quite poorly for Cloverleaf3D
 shows the average participate rate
More exploration by box

More exploration by data set

More exploration by line / plane

Table with avgRankP for the tableau entries.

Box-based tableau.
1 plot per datasets -- All seeding inside of it.
1 line per seeding strategy.
Also do the other: B: (all datasets), etc.
Line/Plane

Section outline:
\begin{itemize}
    \item Describe rank participation: Definition, image of several rank participations.
    \item Table contains all of the averages for rank P.
    \item discuss use cases: FTLE, streamline, Poincare. 
    \begin{itemize} 
    \item Consider adding a fusion/syn poincare case with many more steps. 10k, 20k, 50k, 100k
    \end{itemize}
    \item Performance from a box-centric perspective:
    \begin{itemize}
        \item Whole and Large box: good to ok for small number of steps.  Avgs= .723 and .620 respectively.
        \item RP drops off significantly after Box50
        \item Fusion and synthetic and why they do well with B,B50 and then drop off.
    \end{itemize}
    \item Performance from a DS perspective
    \begin{itemize}
        \item RP dropoff rates. Clustering of lines: supernova 2 clusters, tokamak 2, syn 2, hyrdo ? cloverleaf 2 towards the end. cloverleaf seems to converge.  Do they all converge? They seem to..  
    \end{itemize}
    \item Performance that is being left on the table. 
    \item We need to look at RP for other algorithms and compare.
    \item RP and Time may be in tension. RP of 1.0 but time of 3X is no good... Do we need a RP vs. Time chart?  Have clover Scatter plots.  Add a plot for Avg Time vs. Avg RP for each seeding strategy.
\end{itemize}
\fi










\if 0

\begin{figure*}[ht]
\centering
\subfigure[Astro]{
\label{fig:dscentric:astro}  \includegraphics[width=55mm]{./figs/DSCentric/astro}}
\subfigure[Fusion]{\label{fig:dscentric:fusion}  \includegraphics[width=55mm]{./figs/DSCentric/fusion}}
\subfigure[Fishtank]{\label{fig:dscentric:fishtank}  \includegraphics[width=55mm]{./figs/DSCentric/fishtank}}
\\
\subfigure[Cloverleaf]{\label{fig:dscentric:clover}  \includegraphics[width=55mm]{./figs/DSCentric/clover}}
\subfigure[Synthetic]{\label{fig:dscentric:syn}  \includegraphics[width=55mm]{./figs/DSCentric/syn}}
\caption{Dataset centric plots}
\label{fig:datasets}
\end{figure*}

\begin{figure*}[ht]
\centering
\subfigure[Whole Box]{
\label{fig:boxcentric:B}  \includegraphics[width=55mm]{./figs/BoxCentric/B}}
%
\subfigure[Box 50]
{\label{fig:boxcentric:B0}  \includegraphics[width=55mm]{./figs/BoxCentric/B0}}
%
\subfigure[Box 25]
{\label{fig:boxcentric:B1}  \includegraphics[width=55mm]{./figs/BoxCentric/B1}}

\subfigure[Box 10]
{\label{fig:boxcentric:B2}  \includegraphics[width=55mm]{./figs/BoxCentric/B2}}
%
\subfigure[Box 5]
{\label{fig:boxcentric:B3}  \includegraphics[width=55mm]{./figs/BoxCentric/B3}}
\caption{Seeding volume centric plots}
\label{fig:seed-boxes}
\end{figure*}
\fi



\if 0

\begin{table}[htb]
\begin{center}
\caption {Rank Participation averages.}
\label{table:allAvgs}
\begin{tabular}{llllllll|l}
\multicolumn{1}{l|}{\textbf{Dataset}} &
  \textbf{Whole Box} &
  \textbf{Box 50} &
  \textbf{Box 25} &
  \textbf{Box 10} &
  \textbf{Box 5} &
  \textbf{Line} &
  \textbf{Plane} &
  \textbf{Avg (no L,P)} \\ \cline{1-8}
\multicolumn{1}{l|}{Tokamak}      & 0.835 & .790 & .239 & .241 & .176 & .320 & .407 & .456 \\
\multicolumn{1}{l|}{Supernova}    & 0.614 & .626 & .562 & .630 & .278 & .324 & .482 & .542 \\
\multicolumn{1}{l|}{Hydraulics}   & 0.695 & .390 & .341 & .182 & .143 & .226 & .464 & .350 \\
\multicolumn{1}{l|}{CloverLeaf3D} & 0.547 & .391 & .305 & .188 & .268 & .194 & .327 & .340 \\
\multicolumn{1}{l|}{Synthetic}    & 0.924 & .900 & .170 & .148 & .184 & .758 & .411 & .465 \\ \hline
Avg                               & .723  & .620 & .323 & .278 & .210 & .364 & .418 & .419
\end{tabular}
\end{center}
\end{table}

\fi




